Quantifier Elimination With Structural Learning

We consider the Quantifier Elimination (QE) problem for propositional CNF formulas with existential quantifiers. QE plays a key role in formal verification. Earlier, we presented an approach based on the following observation. To perform QE, one just needs to add a set of clauses depending on free variables that makes the quantified clauses (i.e. clauses with quantified variables) redundant. To implement this approach, we introduced a branching algorithm making quantified clauses redundant in subspaces and merging the results of branches. To implement this algorithm we developed the machinery of D-sequents. A D-sequent is a record stating that a quantified clause is redundant in a specified subspace. Redundancy of a clause is a structural property (i.e. it holds only for a subset of logically equivalent formulas as opposed to a semantic property). So, re-using D-sequents is not as easy as re-using conflict clauses in SAT-solving. In this paper, we address this problem. We introduce a new definition of D-sequents that enables their re-usability. We develop a theory showing under what conditions a D-sequent can be safely re-used.

==> d3ep_sequents_proofs.tex <==
\section*{Propositions of Section~\ref{sec:dseqs}: Dependency Sequents (D-sequents)}




==> f0ootnote.tex <==
A clause is a disjunction of literals. So a CNF formula $F$ is a
conjunction of clauses: $C_1 \wedge \dots \wedge Ck$. We will also
view $F$ just a set of clauses \s{C_1,\dots,C_k}. Given formula
\prob{X}{F} we will say that clause $C$ is redundant in \prob{X}{F} if
$\prob{X}{F} \equiv \prob{X}{F \setminus \s{C}}$.


==> f1ootnote.tex <==
Indeed, $\prob{X}{F^* \wedge F} \equiv \prob{X}{F}$ since $F
\rightarrow F^*$. On the other hand, $\prob{X}{F^* \wedge F} \equiv
\prob{X}{F^*} \equiv F^*$ since adding $F^*$ makes $F$ redundant and
$F^*$ does not depend on $X$.


==> old_files/a2tomic_dseqs.tex <==
\section{Atomic D-sequents}
\label{sec:atom_dseqs}
In this section we describe D-sequents called atomic. These D-sequents
are generated when redundancy of a clause can be trivially
proved. Similarly to~\cite{fmcad13}, we introduce atomic D-sequents of
three kinds. However, in contrast to~\cite{fmcad13}, we consider
D-sequents specified by Definition~\ref{def:dseq}. In particular, we
show that D-sequents of the first kind are robust whereas D-sequents
of the second and third kind are fragile.
%
% Subsection: sat. clause
%
\subsection{Atomic D-sequents of the first kind}
\begin{proposition}
  \label{prop:sat_cls}
 Let \prob{X}{F} be an \ecnf and $C \in F$ and $v \in \V{C}$. Let
 assignment $v=b$ where $b \in \s{0,1}$ satisfy $C$. Then D-sequent
 \ooods{(v=b)}{C} holds. We will refer to it as an atomic D-sequent of
 the \tb{first kind}.
\end{proposition}
%
%  Example
%
\begin{example}
  Let \prob{X}{F} be an \ecnf and $C=\overline{x}_1 \vee y_5$ be a
  clause of $F$.  Since $C$ is satisfied by assignments $x_1 = 0$ and
  $y_5=1$, D-sequents \ooods{(x_1=0)}{C} and \ooods{(y_5=1)}{C} hold.
\end{example}
%
%  Subsection: second kind
%
\subsection{Atomic D-sequents of the second kind}
\label{ssec:second_kind}
%
%
\begin{proposition}
  \label{prop:uns_cls}
 Let \prob{X}{F} be an \ecnf formula and \pnt{q} be an assignment to
 \V{F}.  Let $B,C$ be two clauses of $F$. Let \cof{C}{q} be an
 $X$-clause and \cof{B}{q} imply \cof{C}{q} (i.e. every literal of
 \cof{B}{q} is in \cof{C}{q}). Then the D-sequent \ods{q}{H}{C} holds
 where $H = \s{B}$.  We will refer to it as an atomic D-sequent of the
 \tb{second kind}.
\end{proposition}
%
%
\begin{example}
  Let \prob{X}{F} be an \ecnf formula.  Let $B=y_1 \vee x_2$ and $C =
  x_2 \vee \overline{x}_3$ be $X$-clauses of $F$. Let
  $\pnt{q}=(y_1=0)$.  Since \cof{B}{q} implies \cof{C}{q}, the
  D-sequent \ods{q}{\s{B}}{C} holds. Since \cof{B}{q} \,is an
  $X$-clause, this D-sequent is fragile.
\end{example}

%
% Subsection: third kind
%
\subsection{Atomic D-sequents of the third kind}
\label{ssec:third_kind}
To introduce atomic D-sequents of the third kind, we need to make a
few definitions.
%
% Resolution of clauses
%
\begin{definition}
\label{def:resol}
Let $C'$ and $C''$ be  clauses having opposite
  literals of exactly one variable $v \in \V{C'} \cap \V{C''}$. 
The clause $C$ consisting of all literals of $C'$ and $C''$ but
those of $v$ is called the \tb{resolvent} of $C'$,$C''$ on $v$.
Clause $C$ is said to be obtained by \tb{resolution} on $v$.
Clauses $C'$,$C''$ are called \tb{resolvable} on $v$.
\end{definition}
%
%  blocked clause
%
\begin{definition}
\label{def:blk_cls}
 A clause $C$ of a CNF formula $F$ is called \tb{blocked} at variable
 $v$, if no clause of $F$ is resolvable with $C$ on $v$.  The notion
 of blocked clauses was introduced in~\cite{blocked_clause}.
\end{definition}

%
% Proposition: Dseq of the third kind
%
\begin{proposition}
  \label{prop:dseq_third_kind}
Let \prob{X}{F} be an \ecnf formula. Let $C$ be an $X$-clause of $F$
and $v \in\V{C} \cap X$. Let $C_1,\dots,C_k$ be the clauses of $F$
that can be resolved with $C$ on variable $v$. Let
\noDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$,\noDs{\ppnt{q}{k}}{H_k}{C_k} be a
consistent set\footnote{\input{f9ootnote}} of D-sequents.  Then
D-sequent \noDs{q}{H}{C} holds where
\pnt{q}=$\bigcup\limits_{i=1}^{i=k}\ppnt{q}{i}$ and $H =
\bigcup\limits_{i=1}^{i=k}H_i$. We will refer to it as an atomic
D-sequent of the \tb{third kind}.
\end{proposition}

Note that, in general, a D-sequent of the third kind is fragile.

%
%  Example
%
\begin{example}
  Let \prob{X}{F(X,Y)} be an \ecnf formula. Let $C_3,C_6,C_8$ be the
  only clauses of $F$ with variable $x_5 \in X$ where $C_3 = x_5
  \wedge x_{10} $, $C_6 = \overline{x}_5 \wedge y_1$, $C_8 =
  \overline{x_5} \vee y_3 \vee y_5$. Note that assignment $y_1=1$
  satisfies clause $C_6$.  So the D-sequent \ooods{(y_1=1)}{C_6}
  holds. Suppose that D-sequent \noDs{\pnt{r}}{\s{C_{10}}}{C_8} holds
  where $C_{10}$ is a clause of $F$ and $\pnt{r} = (y_2=0,x_{10}=1)$.
  From Proposition~\ref{prop:dseq_third_kind} it follows that
  D-sequent \noDs{\pnt{q}}{\s{C_{10}}}{C_3} holds where $\pnt{q} =
  (y_1=1,y_2=0,x_{10}=1)$.
\end{example}



==> old_files/a3tomic_dseqs_proofs.tex <==
\section*{Propositions of Section~\ref{sec:atom_dseqs}: Atomic D-sequents}
%
% Proposition: Dseq of the first kind
%
\begin{proposition}
%  \label{prop:sat_cls}
  Let \prob{X}{F} be an \ecnf. Let $v \in \V{C}$ and by assigning
  value $b$ to $v$ where $b \in \s{0,1}$ one satisfies $C$. Then
  D-sequent \ooods{(v=b)}{C} holds We will refer to it as a
  \tb{D-sequent of the first kind}.
\end{proposition}  
\begin{mmproof}
  Let \pnt{q} denote $(v=b)$. Let $W$ be a member formula for the
  D-sequent \ooods{(v=b)}{C}. Hence, $W$ contains $C$. Clause
  \cof{C}{q} is \ti{true} and so is redundant in \cof{W}{q} and hence,
  in \prob{X}{\cof{W}{q}}.  $\square$
\end{mmproof}


%
%  Proposition: dseq of the second kind
%
\begin{proposition}
%  \label{prop:uns_cls}
  Let \prob{X}{F} be an \ecnf formula and \pnt{q} be an assignment to
  \V{F}.  Let $B,C$ be two clauses of $F$. Let \cof{C}{q} be an
  $X$-clause and \cof{B}{q} imply \cof{C}{q} (i.e. every literal of
  \cof{B}{q} is in \cof{C}{q}). Then the D-sequent \ods{q}{H}{C} holds
  where $H = \s{B}$ if \cof{B}{q} is an $X$-clause and $H = \emptyset$
  otherwise.  We will refer to the D-sequent above as an atomic
  D-sequent of the \tb{second kind}.
\end{proposition}
%
\begin{mmproof}
 Let $W$ be a member formula for the D-sequent \ods{q}{H}{C}. Then
 $\s{B,C} \subseteq W$. Indeed, if \cof{B}{q} is an $X$-clause then $B
 \in H$ and $H \subseteq W$. Otherwise, $B$ is in $W$ because $W$ is
 obtained from $F$ by removing only clauses that are $X$-clauses in
 subspace \pnt{q}.  Since \cof{B}{q} implies \cof{C}{q}, then
 $\cof{W}{q} \equiv \cof{W}{q} \setminus \s{\cof{C}{q}}$.$\square$
\end{mmproof}

%
%  Lemma: Blocked clause
%
\begin{lemma}
\label{lem:blk_cls}
Let \prob{X}{F} be an \ecnf formula and \pnt{q} be an assignment to
\V{F}. Let $C$ be an $X$-clause of $F$ not satisfied by \pnt{q} and $v
\in X$ be a variable of $C$ such that $v \not\in \Va{q}$.  Let clause
\cof{C}{q} be blocked at $v$ in \cof{F}{q}.  Then \cof{C}{q} is
redundant in \prob{X}{\cof{F}{q}}.
\end{lemma}
\begin{mmproof}
Assume the contrary i.e. \cof{C}{q} is not redundant in
\prob{X}{\cof{F}{q}}. Then there is a $Z$-boundary point \pnt{p} where
$Z \subseteq X$ that falsifies only \cof{C}{q} and is $X$-removable in
\cof{F}{q}. Let \pnt{p'} be the point obtained from \pnt{p} by
flipping the value of $v$. Consider the following two possibilities.
\begin{itemize}
\item \pnt{p'} satisfies \cof{F}{q}. Then \pnt{p} is not
 $X$-removable and we have a contradiction.
\item \pnt{p'} falsifies a clause \cof{C'}{q} of \cof{F}{q}. Then
  \cof{C}{q} and \cof{C'}{q} are resolvable on variable $v$ and we
  have a contradiction again. $\square$
\end{itemize}
\end{mmproof}


%
% Proposition: Dseq of the third kind
%
\begin{proposition}
%  \label{prop:dseq_third_kind}
Let \prob{X}{F} be an \ecnf formula. Let $C$ be an $X$-clause of $F$
and $v \in\V{C} \cap X$. Let $C_1,\dots,C_k$ be the clauses of $F$
that can be resolved with $C$ on variable $v$. Let
\noDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$,\noDs{\ppnt{q}{k}}{H_k}{C_k} be a
consistent set of D-sequents.  Then D-sequent \noDs{q}{H}{C} holds
where \pnt{q}=$\bigcup\limits_{i=1}^{i=k}\ppnt{q}{i}$ and $H =
\bigcup\limits_{i=1}^{i=k}H_i$. We will refer to it as an atomic
D-sequent of the \tb{third kind}.
\end{proposition}
%
\begin{mmproof}
  Let $W$ be a member formula for the D-sequent \noDs{q}{H}{C}.  Since
  $H_i \subseteq H$ holds, $W$ is a member formula for D-sequent
  \noDs{\ppnt{q}{i}}{H_i}{C_i} too. So $C_i$ is redundant in
  \prob{X}{W} in subspace \ppnt{q}{i}.  Since $\ppnt{q}{i} \subseteq
  \pnt{q}$, from Proposition~\ref{prop:subspace} it follows, that
  $C_i$ is redundant in \prob{X}{W} in subspace \pnt{q} too. Since
  D-sequents \noDs{\ppnt{q}{1}}{H_1}{C_1}, $\dots$,
  \noDs{\ppnt{q}{k}}{H_k}{C_k} are consistent, the clauses
  $C_1,\dots,C_k$ are redundant together in \prob{X}{W} in subspace
  \pnt{q}. So clause $C$ is blocked in \prob{X}{W} at variable $v$ in
  subspace \pnt{q}. From Lemma~\ref{lem:blk_cls} it follows that $C$
  is redundant in \prob{X}{W} in subspace \pnt{q}.  $\square$
\end{mmproof}


==> old_files/abstract.tex <==
\begin{abstract}
  We consider the Quantifier Elimination (QE) problem for
  propositional CNF formulas with existential quantifiers.  QE plays a
  key role in formal verification. Earlier, we presented an approach
  based on the following observation. To perform QE, one just needs to
  add a set of clauses depending on free variables that makes the
  quantified clauses (i.e. clauses with quantified variables)
  redundant.  To implement this approach, we introduced a branching
  algorithm making quantified clauses redundant in subspaces and
  merging the results of branches. To implement this algorithm we
  developed the machinery of D-sequents. A D-sequent is a record
  stating that a quantified clause is redundant in a specified
  subspace. Redundancy of a clause is a structural property (i.e. it
  holds only for a \ti{subset} of logically equivalent formulas as
  opposed to a \ti{semantic} property). So, re-using D-sequents is not
  as easy as re-using conflict clauses in SAT-solving. In this paper,
  we address this problem. We introduce a new definition of D-sequents
  that enables their re-usability. We develop a theory showing under
  what conditions a D-sequent can be safely re-used.
\end{abstract}




==> old_files/b0asic.tex <==
%\section{Redundant Clauses, Boundary Points, And Quantifier Elimination}
\section{Basic Definitions}
\label{sec:basic}

In this paper, we consider only propositional CNF formulas. In the
sequel, when we say ``formula'' without mentioning quantifiers we mean
a quantifier-free CNF formula.  We consider \ti{true} and \ti{false}
as a special kind of clauses. A non-empty clause $C$ becomes \ti{true}
when it is satisfied by an assignment \pnt{q} \,i.e. when a literal of
$C$ is set to \ti{true} by \pnt{q}. A clause $C$ becomes \ti{false}
when it is falsified by \pnt{q} i.e.  when all the literals of $C$ are
set to \ti{false} by \pnt{q}.
%
%  Ecnf
%
\begin{definition}
 \label{def:ecnf}
  Let $F$ be a CNF formula and $X$ be a subset of variables of $F$. We
  will refer to formula \prob{X}{F} as \bm{\ecnf}.
\end{definition}
%
%  Vars(F)
%
\begin{definition}
  \label{def:vars}
Let \pnt{q} be an assignment and $F$ be a CNF formula. \bm{\Va{q}}
denotes the variables assigned in \pnt{q}; \bm{\V{F}} denotes the set
of variables of $F$; \bm{\V{\prob{X}{F}}} denotes $\V{F} \setminus X$.
\end{definition}
%
%  Cofactor
%
\begin{definition}
  \label{def:cofactor}
Let $C$ be a clause, $H$ be a formula that may have quantifiers, and
\pnt{p} be an assignment. \bm{\cof{C}{p}} is true if $C$ is satisfied
by \pnt{p}; otherwise it is the clause obtained from $C$ by removing
all literals falsified by \pnt{p}. \bm{\cof{H}{p}} denotes the formula
obtained from $H$ by replacing $C$ with \cof{C}{p}.
\end{definition}
%
%   Formula equivalence
%
\begin{definition}
\label{def:formula-equiv}
Let $G, H$ be formulas that may have quantifiers. We say that $G, H$
are \tb{equivalent}, written \bm{G \equiv H}, if for all assignments
$\pnt{q}$ such that $\Va{q}$ $\supseteq (\V{G} \cup \V{H})$, we have
$\cof{G}{q} = \cof{H}{q}$.
% Notice that if $\Va{q} \subseteq \V{\exists X
%  [F]}$, then $\cof{(\exists X [F])}{q} \equiv \exists X [\cof{F}{q}]$.
\end{definition}
%
%   QE problem
%
\begin{definition}
 \label{def:qe-solution}
The \tb{Quantifier Elimination (QE)} problem for \ecnf formula
\prob{X}{F(X,Y)} is to find a formula $F^*(Y)$ such that \bm{F^*
  \equiv \prob{X}{F}}.
\end{definition}

%
%  Remark
%
\begin{remark}
\label{rem:X_Y_sets}
From now on, we will use $Y$ and $X$ to denote sets of free and
quantified variables respectively. We will assume that variables
denoted by $x_i$ and $y_i$ are in $X$ and $Y$ respectively. When we
use $Y$ and $X$ in a quantifier-free formula we mean that, in the
context of QE, the set $X$ specifies the quantified variables.
\end{remark}
%
% X-clause, non-X-clause
%
\begin{definition}
\label{def:X_clause}
 A clause $C$ of $F$ is called a \bm{Z}\tb{-clause} 
 if \V{C} $\cap~Z~\neq~\emptyset$. Denote by
           {\boldmath $F^{Z}$} the set of all $Z$-clauses of
           $F$.
\end{definition}
%
% redundant clauses
%
\begin{definition}
\label{def:red_cls}
Let $F$ be a CNF formula and $G \subseteq F$ (i.e. G is a non-empty
subset of clauses of $F$).  The clauses of $G$ are \textbf{redundant}
in $F$ if $F \equiv (F \setminus G)$.  The clauses of $G$ are
\textbf{redundant} in formula \prob{X}{F} if $\prob{X}{F} \equiv
\prob{X}{F \setminus G}$.
\end{definition}

Note that $F \equiv (F \setminus G)$ implies $\prob{X}{F} \equiv
\prob{X}{F \setminus G}$ but the opposite is not true.


==> old_files/b1nd_pnts.tex <==
\section{Clause Redundancy And Boundary Points}
\label{sec:bnd_pnts}
In this section, we explain the semantics of QE in terms so-called
boundary points.
%  
% point
%
\begin{definition}
\label{def:pnt}
Given assignment \pnt{p} and a formula $F$, we say that \pnt{p} is a
\textbf{point} of $F$ if $\V{F} \subseteq \Va{p}$.
%if $\V{F} \subseteq \Va{p}$.
\end{definition}

In the sequel, by ``assignment'' we mean a possibly partial one. To
refer to a \ti{full} assignment we will use the term ``point''.

%
% Z-boundary point 
%
\begin{definition}
  \label{def:bnd_pnt}
 Let $F$ be a formula and $Z \subseteq \V{F}$.  A point \pnt{p} of $F$
 is called a \bm{Z}\tb{-boundary point} of $F$ if a) $Z \neq
 \emptyset$ and b) $\cof{F}{p} = \mi{false}$ and c) every clause of
 $F$ falsified by \pnt{p} is a $Z$-clause and d) the previous
 condition breaks for every proper subset of $Z$.
\end{definition}

\begin{remark}
  Let $F(X,Y)$ be a CNF formula where sets $X$ and $Y$ are interpreted
  as described in Remark~\ref{rem:X_Y_sets}. In the context of QE, we
  will deal exclusively with $Z$-boundary points that falsify only
  $X$-clauses of $F$ and so $Z \subseteq X$ holds.
\end{remark}
%
% Example
%
% v1 -> x1, v2->x2, v4->x3
% v3 -> y1, v5 -> y2
\begin{example}
\label{exmp:bnd_pnt}
Let $X = \s{x_1,x_2,x_3}$ and $Y=\s{y_1,y_2}$. Let $F(X,Y)$ be a CNF
formula of four clauses: $C_1 = x_1 \vee x_2$, $C_2 = \overline{x}_1
\vee y_1$, $C_3 = x_1 \vee \overline{x}_3 \vee y_2$, $C_4 =
\overline{x}_2 \vee y_2$. The clauses of $F$ falsified by \pnt{p} =
$(x_1=0,x_2=0,x_3=1,y_1=0,y_2=0)$ are $C_1$ and $C_3$. One can verify
that \pnt{p} and the set $Z= \s{x_1}$ satisfy the four conditions of
Definition~\ref{def:bnd_pnt}, which makes \pnt{p} a \s{x_1}-boundary
point. The set $Z$ above is not unique. One can easily check that
\pnt{p} is also a \s{x_2,x_3}-boundary point.
\end{example}
The term ``boundary'' is justified as follows.  Let $F$ be a
satisfiable CNF formula with at least one clause.  Then there always
exists a \s{v}-boundary point of $F$, $v \in \V{F}$ that is different
from a satisfying assignment only in value of $v$.

%
%  removable boundary points
%
\begin{definition}
\label{def:rem_bnd_pnt}
Given a CNF formula $F(X,Y)$ and a $Z$-boundary point \pnt{p} of $F$:
\begin{itemize} 
\item \pnt{p} is $X'$-\tb{removable} in $F$ if 1) $Z \subseteq X'
  \subseteq X$; and 2) there is a clause $C$ such that a) $F
  \Rightarrow C$; b) $\V{C} \cap X' = \emptyset$; and c)
  $\cof{C}{p} = \mathit{false}$.

\item \pnt{p} is
\tb{removable} in $\prob{X}{F}$ if \pnt{p} is $X$-removable in $F$.
\end{itemize} 
\end{definition}

In the above definition, notice that \pnt{p} is not a $Z$-boundary
point of $F \wedge C$ because \pnt{p} falsifies $C$ and $\V{C}\cap Z =
\emptyset$. So adding clause $C$ to $F$ eliminates \pnt{p} as a
$Z$-boundary point.
%
% Example
%
\begin{example}
Let us consider the \s{x_1}-boundary point \pnt{p} =
$(x_1=0,x_2=0,x_3=1,y_1=0,y_2=0)$ of Example~\ref{exmp:bnd_pnt}. Let
$C$ denote clause $C = y_1 \vee y_2$ obtained\footnote{See
  Definition~\ref{def:resol} of the resolution operation.} by
resolving $C_1$, $C_2$ and $C_4$ on variables $x_1$ and $x_2$.  Note
that set $Z = \s{x_1}$ and $C$ satisfy the conditions a),b) and c) of
Definition~\ref{def:rem_bnd_pnt} for $X' = X$.  So \pnt{p}~~is an
$X$-removable \s{x_1}-boundary point. After adding $C$ to $F$, \pnt{p}
is not an \s{x_1}-boundary point any more. Let us consider the point
\pnt{q}=$(x_1=0,x_2=0,x_3=1,y_1=1,y_2=1)$ obtained from \pnt{p} by
flipping values of $y_1$ and $y_2$. Both \pnt{p} and \pnt{q} have the
same set of falsified clauses consisting of $C_1$ and $C_3$. So, like
\pnt{p}, point \pnt{q} is an \s{x_1}-boundary point. However, no
clause $C$ implied by $F$ and consisting only of variables of $Y$ is
falsified by \pnt{q}. So, the latter, is an \s{x_1}-boundary point
that is \ti{not} $X$-removable.
\end{example}
%
% proposition: removable boundary points
%
\begin{proposition}
\label{prop:rem_bnd_pnt}
A $Z$-boundary point \pnt{p} of $F(X,Y)$ is removable in \prob{X}{F}, iff
one cannot turn \pnt{p} into an assignment satisfying $F$ by changing
only the values of variables of $X$.
\end{proposition}

The proofs are given in the appendix.
%
% proposition : redundant clauses and removable boundary points
%
\begin{proposition}
\label{prop:red_cls_set}
Let $F(X,Y)$ be a CNF formula where $F^X \neq \emptyset$ (see
Definition~\ref{def:X_clause}). Let $G$ be a non-empty subset of
$F^X$.  The set $G$ is not redundant in \prob{X}{F} iff there is a
$Z$-boundary point \pnt{p} of $F$ such that a) every clause falsified
by \pnt{p} is in $G$ and b) \pnt{p} is $X$-removable in $F$.
\end{proposition}

Proposition~\ref{prop:red_cls_set} justifies the following strategy of
solving the QE problem. Add to $F$ a set $G$ of clauses that a) are
implied by $F$; b) eliminate every $X$-removable boundary point
falsifying a subset of $X$-clauses of $F$. By dropping all $X$-clauses
of $F$, one produces a solution to the QE problem.


==> old_files/b2nd_pnts_proofs.tex <==
%\vspace{4pt}
\section*{Propositions of
Section~\ref{sec:bnd_pnts}: Clause Redundancy And Boundary Points}

%
% proposition: removable boundary points
%

\begin{proposition}
%\label{prop:rem_bnd_pnt}
A $Z$-boundary point \pnt{p} of $F(X,Y)$ is removable in \prob{X}{F}, iff
one cannot turn \pnt{p} into an assignment satisfying $F$ by changing
only the values of variables of $X$.
\end{proposition}
%
%
\begin{mmproof} \ti{If part}. Assume the contrary. That is \pnt{p} \,is
not removable while no satisfying assignment can be obtained from
\pnt{p} by changing only values of variables of $X$. Let $C$ be the
clause consisting of all variables of $Y$ and falsified by
\pnt{p}. Since \pnt{p} is not removable, clause $C$ is not implied by
$F$. This means that there is an assignment \pnt{s} that falsifies $C$
and satisfies $F$. By construction, \pnt{s} and \pnt{p} \,have identical
assignments to variables of $Y$. Thus, \pnt{s} can be obtained from
\pnt{p} by changing only values of variables of $X$ and we have a
contradiction.
\vspace{3pt}
%

\noindent\textit{Only if part.} Assume the contrary. That is \pnt{p}
is removable but one can obtain an assignment \pnt{s} satisfying $F$
from \pnt{p} \,by changing only values of variables of $X$.  Since
\pnt{p} \,is removable, there is a clause $C$ that is implied by $F$
and falsified by \pnt{p} and that depends only of variables of
$Y$. Since \pnt{s} and \pnt{p} \,have identical assignments to
variables of $Y$, point \pnt{s} \,falsifies $C$. However, since
\pnt{s} satisfies $F$, this means that $C$ is not implied by $F$ and
we have a contradiction. $\square$
\end{mmproof}


%
% proposition : redundant clauses and removable boundary points
%
\begin{proposition}
%\label{prop:red_cls_set}
Let $F(X,Y)$ be a CNF formula where $F^X \neq \emptyset$ (see
Definition~\ref{def:X_clause}). Let $G$ be a non-empty subset of
$F^X$.  The set $G$ is not redundant in \prob{X}{F} iff there is a
$Z$-boundary point \pnt{p} of $F$ such that a) every clause falsified
by \pnt{p} is in $G$ and b) \pnt{p} is $X$-removable in $F$.
\end{proposition}
%
% Proof
%
\begin{mmproof}
Let $H$ denote $F \setminus G$. Given a point \pnt{p}, let
(\pnt{x},\pnt{y}) specify the assignments of \pnt{p} to the variables
of $X$ and $Y$ respectively. \\
\noindent\textit{If part.} Assume the contrary, \ie 
 there is an $X$-removable point \pnt{p}=(\pnt{x},\pnt{y}) of $F$ but
 $G$ is redundant in \prob{X}{F} and so
 $\prob{X}{F} \equiv \prob{X}{H}$.  Since \pnt{p} \,is a boundary point,
 $F(\pnt{p}) = 0$. Since
\pnt{p} \,is removable, $\cof{(\prob{X}{F})}{y} = 0$. On the other hand,
since \pnt{p} \,falsifies only clauses of $G$ it satisfies $H$.
Hence $\cof{(\prob{X}{H})}{y} = 1$ and
$\cof{(\prob{X}{F})}{y} \neq \cof{(\prob{X}{H})}{y}$, which leads to a
contradiction.

\vspace{3pt}
\noindent\textit{Only if part.}  Assume the contrary, \ie set $G$ is
not redundant (and hence $\prob{X}{F} \not\equiv \prob{X}{H}$) and
there does not exist an $X$-removable $Z$-boundary point of $F$
falsifying only clauses of $G$.  Let \pnt{y} be an assignment to $Y$
such that $\cof{(\prob{X}{F})}{y} \neq \cof{(\prob{X}{H})}{y}$.
Consider the following two cases.
\begin{itemize}
%
\item   $\cof{(\prob{X}{F})}{y}=1$ and $\cof{(\prob{X}{H})}{y}=0$.
Then there exists an assignment \pnt{x} to $X$ such that
(\pnt{x},\pnt{y}) satisfies $F$. Since every clause of $H$ is in $F$,
formula $H$ is also satisfied by \pnt{p}. So we have a contradiction.
%
\item $\cof{(\prob{X}{F})}{y}=0$ and $\cof{(\prob{X}{H})}{y}=1$. Then
  there exists an assignment \pnt{x} to variables of $X$ such that
  (\pnt{x},\pnt{y}) satisfies $H$.  Since $\cof{F}{y} \equiv 0$, point
  (\pnt{x},\pnt{y}) falsifies $F$. Since $H(\pnt{p})=1$,
  (\pnt{x},\pnt{y}) is a $Z$-boundary point of $F$ that falsifies only
  clauses of $G$.  Since $\cof{F}{y} \equiv 0$, (\pnt{x},\pnt{y}) is
  an $X$-removable $Z$-boundary point of $F$, which leads to a
  contradiction.~$\square$
\end{itemize}
\end{mmproof}


==> old_files/commands.tex <==
%
%
%
%
%
\newcommand{\jd}{\mbox{$\mi{JoinDseqs}$}\xspace}
\newcommand{\Jd}{\mbox{$\mi{JoinDseqs}^+$}\xspace}
\newcommand{\Di}{$\mi{DDS}~$}
\newcommand{\cdi}{\mbox{$\mi{DCDS}$}\xspace}
\newcommand{\Cdi}{\mbox{$\mi{DCDS^+}$}\xspace}
\newcommand{\PS}{\mbox{$\Psi$}\xspace}
\newcommand{\FI}{\mbox{$\Phi$}\xspace}
\newcommand{\olds}[4]{\mbox{$(\prob{#1}{#2},\pnt{#3})~\rightarrow #4$}}
\newcommand{\Ods}[5]{\mbox{$(\prob{#1}{#2},\pnt{#3},#4)~\rightarrow #5$}}
\newcommand{\ODs}[5]{\mbox{$(\prob{#1}{#2},#3,#4)~\rightarrow #5$}}
\newcommand{\ods}[3]{\mbox{$(\pnt{#1},#2)~\rightarrow #3$}}
\newcommand{\nods}[3]{$(\pnt{#1},#2)~\rightarrow #3$}
\newcommand{\oDs}[3]{\mbox{$(#1,#2)~\rightarrow #3$}}
\newcommand{\noDs}[3]{$(#1,#2)~\rightarrow #3$}
\newcommand{\oods}[2]{\mbox{\pnt{#1}~$\rightarrow #2$}}
\newcommand{\ooods}[2]{\mbox{$#1 \rightarrow #2$}}
\newcommand{\Uds}[4]{\mbox{$(\prob{#1}{#2},\pnt{#3})\rightarrow #4$}}
\newcommand{\uds}[4]{\mbox{$(\prob{#1}{#2},#3)\rightarrow #4$}}
%
%
\newenvironment{mproof}{\hspace{8pt}\ti{Proof:}}{~~~~QED}
\newenvironment{mmproof}{\hspace{8pt}\ti{Proof:}}{}
%\newcommand{\ie}{\emph{i.e.}, }
%\newcommand{\eg}{\emph{e.g.}, }
\newcommand{\ie}{i.e., }
\newcommand{\eg}{e.g., }
\newcommand{\pnt}[1]{{\mbox{$\vec{#1}$}}}
\newcommand{\ppnt}[2]{{\mbox{$\vec{#1}_{#2}$}}}
\newcommand{\pppnt}[2]{{\mbox{$\vec{#1}#2$}}}
\newcommand{\bm}[1]{{\mbox{\boldmath $#1$}}}
%\newcommand{\ppnt}[2]{{\mbox{\boldmath $#1_{#2}$}}}
\newcommand{\cof}[2]{\mbox{$#1_{\vec{#2}}$}}
\newcommand{\coff}[2]{$#1_{\mbox{\boldmath $#2$}}$}
\newcommand{\lit}[2]{\textit{lit}($#1_{#2}$)}  
\newcommand{\tho}{\footnotesize{1000}}
\newcommand{\A}[1]{\ti{\small{Assigned}}(\pnt{q},$#1$)}
\newcommand{\F}[1]{\ti{\footnotesize{Done}}(\pnt{q},$#1$)}
\newcommand{\V}[1]{\mbox{$\mathit{Vars}(#1)$}}
\newcommand{\Va}[1]{\mbox{$\mathit{Vars}(\vec{#1})$}}
\newcommand{\Vaa}[1]{\mathit{Vars}(\boldsymbol{#1})}
\newcommand{\Cls}[1]{\mbox{$\mathit{Clauses}(#1)$}}
\newcommand{\sx}{\mbox{$\{x\}$}}
\newcommand{\s}[1]{\mbox{$\{#1\}$}}
\newcommand{\mvar}{\mbox{$|\mathit{Vars}(F)| + 1$}}
\newcommand{\Gz}[2]{$#1_{\{#2\}}$}
\newcommand{\nGz}[2]{$G_{non-\{z\}}$}
\newcommand{\Ex}[2]{$\mathit{Exst}(#1,#2)$}
\newcommand{\Exo}[2]{$\mathit{Exst}$(#1,$#2$)}
\newcommand{\Dis}[2]{\mbox{$#1 \setminus #2$}}
\newcommand{\DDis}[3]{\mbox{$\cof{#1}{#2} \setminus {#3}$}}
\newcommand{\pr}[1]{\mbox{$\mathit{Prev}$(\pnt{#1})}}
\newcommand{\prr}[1]{\mi{Prev}(\boldsymbol{q})}
\newcommand{\la}[1]{\mbox{$\mathit{Last}$(\pnt{#1})}}
\newcommand{\Bd}[2]{\mbox{$\mathit{Bd}(\pnt{#1},#2)$}}
\newcommand{\Bdl}[1]{\mbox{$\mathit{Bd}(\pnt{#1})$}}
\newcommand{\Dp}[2]{\mbox{$\mathit{Depth}(\pnt{#1},#2)$}}
\newcommand{\Dpl}[1]{\mbox{$\mathit{Depth}$(\pnt{#1})}}
\newcommand{\Sm}[2]{\mbox{$\mathit{Sym}(\pnt{#1},#2)$}}
\newcommand{\re}[2]{\mbox{$\mathit{rec\_lev}(\pnt{#1},#2)$}}
\newcommand{\Nd}[1]{\mbox{$\mathit{Node}$(\pnt{#1})}}
\newcommand{\Ndd}[1]{\mbox{$\mathit{Node}(#1)$}}
\renewcommand{\labelitemi}{$\bullet$}
\renewcommand{\labelitemiii}{$\bullet$}
\renewcommand{\labelitemiv}{$\bullet$}
\newcommand{\mi}[1]{\mathit{#1}}
\newcommand{\ti}[1]{\textit{#1}}
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\fl}[2]{\mbox{$\mathit{first\_left}(\pnt{#1},#2)$}}
\newcommand{\meq}{$\exists{X}.F(X,Y) \equiv F^*(Y)$~}
\newcommand{\meqq}[1]{$F^*_{#1}(Y_{#1}) \equiv \exists{X_{#1}}.F_{#1}(X_{#1},Y_{#1})$}
\newcommand{\Res}[3]{\mbox{$\mathit{Res}$(\pnt{#1},\pnt{#2},$#3$)}}
\newcommand{\ttt}{\>\>\>}
\newcommand{\tttt}{\>\>\>\>}
\newcommand{\ttttt}{\>\>\>\>\>}
\newcommand{\Tt}{\>\>}
\newcommand{\Sub}[2]{\mbox{$\mi{#1}_\mi{#2}$}}
\newcommand{\sub}[2]{\mbox{$\vec{#1}_\mi{#2}$}}
\newcommand{\Sup}[2]{\mbox{$#1^\mi{#2}$}}
\newcommand{\cc}{\ti{CCR}~}
\newcommand{\Fcurr}{\DDis{F}{q}{\Sub{X}{red}}~}
\newcommand{\Ss}[1]{\scriptsize{#1}}
\newcommand{\Fls}[2]{\mbox{$\mi{FlsCls}(#1,\pnt{#2})$}}
\newcommand{\Nt}[3]{\mbox{$\mi{NonTriv}(#1,#2,#3)$}}
\newcommand{\Xcl}[1]{\mbox{$\mi{Xclauses}(#1)$}}
\newcommand{\Ping}{\mbox{\Sub{P}{ing}}}
\newcommand{\Ped}{\mbox{\Sub{P}{ed}}}
\newcommand{\Prob}[2]{$\exists{#1} [#2]$}
\newcommand{\prob}[2]{\mbox{$\exists{#1} [#2]$}}
\newcommand{\PRob}[3]{\mbox{$\exists{#1}\exists{#2}[#3]$}}
\newcommand{\DS}{\mbox{$\Omega$}\xspace}
\newcommand{\ecnf}{\ensuremath{\exists\mathrm{CNF}}\xspace}
\newcommand{\Comment}[1]{}
\newcommand{\true}{\ensuremath{\mathit{true}}}
\newcommand{\false}{\ensuremath{\mathit{false}}}
\newcommand{\Impl}[2]{\mbox{$#1 \rightarrow #2$}}
\newcommand{\Nmpl}[2]{\mbox{$#1 \not\rightarrow #2$}}
\newcommand{\EC}{\ti{EC\_LoR}~}
\newcommand{\ec}{\ti{EC\_LoR}}
\newcommand{\ECF}{$\mi{EC\!\_LoR}_1$~}
\newcommand{\ecf}{$\mi{EC\!\_LoR}_1$}
\newcommand{\ECS}{$\mi{EC\!\_LoR}_2$~}
\newcommand{\ecs}{$\mi{EC\!\_LoR}_2$}
\newcommand{\tl}[1]{\mbox{$\mi{TopLvl}(#1)$}}
\newcommand{\Pqe}[4]{\mbox{{$#2 \wedge \prob{#1}{#4} \equiv \prob{#1}{#3 \wedge #4}$}}}
\newcommand{\pqe}[4]{$#2 \wedge \prob{#1}{#4} \equiv \prob{#1}{#3 \wedge #4}$}
\newcommand{\SUB}[2]{\mbox{{\boldmath $#1$}$\!_\mi{#2}$}}
\newcommand{\abs}[1]{\mbox{$\mathbb{#1}$}}
\newcommand{\Abs}[2]{\mbox{$\mathbb{#1}_{#2}$}}


==> old_files/d0iv_conq.tex <==
\section{Quantifier Elimination By Branching} 
\label{sec:div_conq}
In this section, we explain the semantics of QE algorithm called
\cdi~\cite{fmcad13} (Derivation of Clause D-Sequents). A high-level
description of \cdi is given in Section~\ref{sec:dcds_recall}. \cdi is
a branching algorithm. Given a formula \prob{X}{F}, \cdi branches on
variables of $F$ until it proves that every $X$-clause is redundant in
the current subspace. (In case of a conflict, proving $X$-clauses of
$F$ redundant, in general, requires adding to $F$ a conflict clause.)
Then \cdi merges the results obtained in different branches to prove
that the $X$-clauses are redundant in the entire search space.  Below
we give propositions justifying the strategy of
\cdi. Proposition~\ref{prop:glb_to_loc} shows how to perform
elimination of removable boundary points of $F$ in the subspace
specified by assignment \pnt{q}. This is done by using formula
\cof{F}{q}, a ``local version'' of $F$.
Proposition~\ref{prop:elim_incr} justifies proving redundancy of
$X$-clauses of \cof{F}{q} incrementally.


%
% Operations on partial assignments
%
Let \pnt{q} and \pnt{r} be assignments to a set of variables $Z$.
Since \pnt{q} and \pnt{r} are sets of value assignments to individual
variables of $Z$ one can apply set operations to them. We will denote
by $\pnt{r} \subseteq \pnt{q}$ the fact that \pnt{q} contains all
value assignments of \pnt{r}.  The assignment consisting of value
assignments of \pnt{q} and \pnt{r} is represented as $\pnt{q} \cup
\pnt{r}$.


%
%  Proposition: globally removable means locally removable
%
\begin{proposition}
\label{prop:glb_to_loc}
Let \prob{X}{F(X,Y)} be an \ecnf and \pnt{q} be an assignment to
\V{F}. Let \pnt{p} be a $Z$-boundary point of $F$ where $\pnt{q}
\subseteq \pnt{p}$ and $Z \subseteq X$. Then if \pnt{p} is removable
in \prob{X}{F} it is also removable in \prob{X}{\cof{F}{q}}.
\end{proposition}
%
% Remark
%
\begin{remark}
\label{rem:no_reverse}
One cannot reverse Proposition~\ref{prop:glb_to_loc}: a boundary point
may be $X$-removable in \cof{F}{q} and not $X$-removable in $F$.  For
instance, if $X=\V{F}$, a $Z$-boundary point \pnt{p} of $F$ where
$|Z|=1$ is removed from \prob{X}{F} only by adding an empty clause to
$F$. So if $F$ is satisfiable, \pnt{p} is not removable. Yet \pnt{p}
may be removable in \prob{X}{\cof{F}{q}} if \cof{F}{q} is
unsatisfiable. A ramification of the fact that
Proposition~\ref{prop:glb_to_loc} is not reversible is discussed in
Section~\ref{sec:virt_red}.

\end{remark}

%
% Proposition: elimination of boundary points incrementally
%
\begin{proposition}
\label{prop:elim_incr}
Let \prob{X}{F(X,Y)} be an \ecnf and $H \subset F^X$ be redundant in
\prob{X}{F}.  Let an $X$-clause $C$ of $F \setminus H$ be redundant in
\prob{X}{F \setminus H}. Then $H \cup \s{C}$ is redundant in
\prob{X}{F}.
\end{proposition}

%
% Remark: redundancy in subspace \pnt{q}
%
\begin{remark}
  \label{rem:red_subsp}
  To simplify the notation, we will sometimes use the expression
  ``clause $C$ is redundant in \prob{X}{F} in subspace \pnt{q}~''
  instead of saying ``clause \cof{C}{q} is redundant in
  \prob{X}{\cof{F}{q}}''.
\end{remark}

Proposition~\ref{prop:elim_incr} shows that one can prove redundancy
of, say, a set of $X$-clauses \s{C',C''} in \prob{X}{F} in subspace
\pnt{q} \ti{incrementally}.  This can be done by a) proving redundancy
of $C'$ in \prob{X}{F} in subspace \pnt{q} and c) proving redundancy
of $C''$ in formula $\prob{X}{F \setminus \s{C'} }$ in subspace
\pnt{q}.


==> old_files/d1iv_conq_proofs.tex <==
\section*{Propositions of Section~\ref{sec:div_conq}: Quantifier Elimination By Branching}
%
%  Proposition: removable in F means removable in \cof{F}{q}
%
\begin{proposition}
%\label{prop:glb_to_loc}
Let \prob{X}{F(X,Y)} be an \ecnf and \pnt{q} be an assignment to
\V{F}. Let \pnt{p} be a $Z$-boundary point of $F$ where $\pnt{q}
\subseteq \pnt{p}$ and $Z \subseteq X$. Then if \pnt{p} is removable
in \prob{X}{F} it is also removable in \prob{X}{\cof{F}{q}}.
\end{proposition}
%
%  Proof
%
\begin{mmproof}
Assume the contrary. That is \pnt{p} is removable in $\prob{X}{F}$ but
is not removable in \prob{X}{\cof{F}{q}}. The fact that \pnt{p} is
removable in \prob{X}{F} means that there is a clause $C$ implied by
$F$ and falsified by \pnt{p} that consists only of variables of $Y$.
Since \pnt{p} is not removable in \prob{X}{\cof{F}{q}}, from
Proposition~\ref{prop:rem_bnd_pnt} it follows that an assignment
\pnt{s} satisfying \cof{F}{q} can be obtained from \pnt{p} by changing
only values of variables of $X \setminus \Va{q}$.  By construction,
\pnt{p} and \pnt{s} have identical assignments to variables of $Y$. So
\pnt{s} has to falsify $C$. On the other hand, by construction,
$\pnt{q} \subseteq \pnt{s}$.  So, the fact that \pnt{s} satisfies
\cof{F}{q} implies that \pnt{s} satisfies $F$ too. Since \pnt{s}
falsifies $C$ and satisfies $F$, clause $C$ is not implied by $F$ and
we have a contradiction. $\square$
\end{mmproof}

% 
% Proposition: elimination of boundary points clause by clause
%
\begin{proposition}
  %\label{prop:elim_incr}  
Let \prob{X}{F(X,Y)} be an \ecnf and $H \subset F^X$ be redundant in
\prob{X}{F}.  Let an $X$-clause $C$ of $F \setminus H$ be redundant in
\prob{X}{F \setminus H}. Then $H \cup \s{C}$ is redundant in
\prob{X}{F}.
\end{proposition}
%
% proof
%
\begin{mmproof}
  Denote $H \cup \s{C}$ as $H'$.  Assume the contrary, i.e.  $H'$ is
  not redundant in \prob{X}{F}. Then, from
  Proposition~\ref{prop:red_cls_set}, it follows that $F$ has an
  $X$-removable boundary \pnt{p} \,such that every clause falsified by
  \pnt{p} \,is in $H'$. Denote as $H''$ the subset of clauses of $H'$
  falsified by \pnt{p}.  Let us consider the two possible cases.
  %
  \begin{itemize}
    %
  \item Clause $C$ is not in $H''$. In this case, $H''$ is a subset of
    $H$ and the existence of \pnt{p} means that $H$ is not
    redundant in \prob{X}{F}. So we have a contradiction.
    %
  \item Clause $C$ is in $H''$. Redundancy of $C$ in \prob{X}{F
    \setminus H} means that one can turn \pnt{p} \,into an assignment
    \pnt{s} satisfying $F \setminus H$ by flipping values of variables
    from $X$. Since \pnt{p} \,is $X$-removable, \pnt{s} \,falsifies
    $F$. The only clauses of $F$ falsified by \pnt{s} are those of
    $H$. Since \pnt{p} and \pnt{s} \,have identical values assigned to
    $Y$, point \pnt{s} \,is $X$-removable as well.  Then the existence
    of \pnt{s} \,means that $H$ is not redundant in \prob{X}{F} and we
    have a contradiction.  $\square$
  \end{itemize}

\end{mmproof}



==> old_files/d2ep_sequents.tex <==
\section{Dependency Sequents (D-sequents)}
\label{sec:dseqs}
In this section, we give a new definition of D-sequents that is
different from that of~\cite{fmcad13}.

%
%  D-sequent
%
\begin{definition}
\label{def:dseq}
Let \prob{X}{F} be an \ecnf formula. Let \pnt{q} be an assignment to
\V{F} and $H \subseteq F^X$ and $C \in F^X$ where $C \not\in H$.  A
dependency sequent (\tb{D-sequent}) $S$ has the form
\Ods{X}{F}{q}{H}{C}. It states that clause \cof{C}{q} is redundant in
every formula \prob{X}{\cof{W}{q}} logically equivalent to
\prob{X}{\cof{F}{q}} where \mbox{$H \cup \s{C} \subseteq W$} and $W
\subseteq F$.  The assignment \pnt{q} and formula $H$ are called the
\tb{conditional} and \tb{order constraint} of $S$ respectively. We
will refer to $W$ as a \tb{member formula} for $S$.
\end{definition}

Definition~\ref{def:dseq} implies that the D-sequent $S$ becomes
inapplicable if a clause of $H$ is removed from $F$. So, $S$ is meant
to be used in situations where the $X$-clauses of $H$ are proved
redundant \ti{after} $C$ (hence the name ``order constraint'').
In~\cite{fmcad13}, a D-sequent specifies redundancy of $C$ in \ti{one
  particular formula} \prob{X}{F}. Adding an order constraint broadens
the set of formulas where $C$ is claimed to be redundant.  We will say
that a D-sequent \Ods{X}{F}{q}{H}{C} is \tb{fragile} if $H$ contains
at least one $X$-clause.  Such a D-sequent becomes inapplicable if an
$X$-clause of $H$ is proved redundant before $C$. If $H$ does not
contain $X$-clauses, the D-sequent above is called \tb{robust}. A
robust D-sequent is not affected by the order in which $X$-clauses are
proved redundant.


%
%  Remark: short notation
%
\begin{remark}
\label{rem:short_dseqs}
We will abbreviate D-sequent \Ods{X}{F}{q}{H}{C} to \ods{q}{H}{C} if
formula \prob{X}{F} is known from the context. We will further reduce
\ods{q}{H}{C} to \oods{q}{C} if $H = \emptyset$ i.e. if no order
constraint is imposed.
\end{remark}


There are two ways to produce D-sequents. First, one can generate an
``atomic'' D-sequent that states a trivial case of redundancy.  The
three atomic types of D-sequents are presented in
Section~\ref{sec:atom_dseqs}. Second, one can use a pair of existing
D-sequents to generate a new one by applying a resolution-like
operation called \ti{join} (Section~\ref{sec:join_dseqs}).





==> old_files/d3ep_sequents_proofs.tex <==
\section*{Propositions of Section~\ref{sec:dseqs}: Dependency Sequents (D-sequents)}




==> old_files/d4cds_alg.tex <==
\section{Recalling \cdi}
\label{sec:dcds_recall}
In~\cite{fmcad13}, we described a QE algorithm called \cdi (Derivation
of Clause D-Sequents) that did not re-use D-sequents. We Recall \cdi in
Subsections~\ref{ssec:dcds} and~\ref{ssec:dcds_corr}.  

%
% Subsection: DCDS
%
\subsection{A brief description of \cdi}
\label{ssec:dcds}



The pseudocode of \cdi is given\footnote{\input{f5ootnote}} in
Fig.~\ref{fig:dcds}. \cdi uses the old definition of a D-sequent
lacking an order constraint. \cdi accepts three parameters: formula
\prob{X}{F} (denoted as \FI), the current assignment \pnt{q} \,and the
set of active D-sequents \DS. (If an $X$-clause of $F$ is proved
redundant in subspace \pnt{q}, this fact is stated by a D-sequent.
This D-sequent is called \tb{active}). \cdi returns the final formula
\prob{X}{F} (where $F$ consists of the initial clauses and derived
clauses implied by $F$) and the set \DS of current active D-sequents.
\DS has an active D-sequent for every $X$-clause of $F$. The
conditional of this D-sequent is a subset of \pnt{q}. In the first
call of \cdi, the initial formula \prob{X}{F} is used and \pnt{q} and
\DS are empty sets. A solution $F^*(Y)$ to the QE problem at hand is
obtained by dropping the $X$-clauses of the final formula \prob{X}{F}
and removing the quantifiers.



\cdi starts with examining the $X$-clauses whose redundancy is not
proved yet.  Namely, \cdi checks if the redundancy of such clauses can
be established by atomic D-sequents (line 1) introduced in
Section~\ref{sec:atom_dseqs}. If all $X$-clauses are proved redundant,
\cdi terminates returning the current formula \prob{X}{F} and the
current set of active D-sequents (lines 2-3). Otherwise, \cdi moves to
the branching part of the algorithm (lines 4-9).

\input{d5cds.fig}

First, \cdi picks a variable $v$ to branch on (line 4). Then it
explores the branch $\pnt{q} \cup \s{v = 0}$ (line 5). The set $\DS_0$
returned in this branch, in general, contains D-sequents whose
conditionals include assignment $v=0$. These D-sequents are
inapplicable in branch $v=1$ and so they are discarded (line 6). After
that \cdi explores branch $\pnt{q} \cup \s{v = 1}$ (line 7) returning
a set of D-sequents $\DS_1$.  Then \cdi generates a set of D-sequents
\DS whose conditionals do not depend on $v$ (line 8). Set \DS consists
of two parts. The first part comprises of the D-sequents of $\DS_0$
that do not depend on $v$. The second part consists of the D-sequents
obtained by joining D-sequents of $\DS_0$ and $\DS_1$ that do depend
on $v$. Finally, \cdi terminates returning \prob{X}{F} and \DS.



%
% Subsection: No D-sequent re-using by DCDS
%
\subsection{Correctness of DCDS}
%\subsection{No D-sequent re-use by \cdi}
\label{ssec:dcds_corr}
As we mentioned above, \cdi is based on D-sequents where no order
constraints are used. So, \cdi cannot check if adding a new D-sequent
to the current set of active D-sequents brings in order-inconsistency.
Hence re-using D-sequents may lead to incorrect results. For that
reason, \cdi just discards the parent D-sequents after the join
operation.

An interesting feature of \cdi is as follows. Assume that one uses the
new definition of D-sequents. That is one adds an order constraint for
an atomic D-sequent of the second/third kind (see
Subsections~\ref{ssec:second_kind} and ~\ref{ssec:third_kind}) and
takes the union of order constraints when performing the join
operation (see Section~\ref{sec:join_dseqs}). Since, in general, the
order in which $X$-clauses are proved redundant in branches $v=0$ and
$v=1$ is different, the set of D-sequents obtained by the \jd
procedure may be inconsistent. However, \cdi is provably
correct\footnote{In~\cite{fmsd14}, we proved the correctness of a
  similar algorithm. This proof applies to \cdi.}. So, the
inconsistency of D-sequents produced by \jd is ``artificial'' and
caused by the imprecision of the joint operation (see
Remark~\ref{rem:ord_constr}).

\input{d6cds+.fig}



==> old_files/d5cds.fig.tex <==
%
%
% DCDS
%
\setlength{\intextsep}{2pt}
\setlength{\textfloatsep}{5pt}
\begin{wrapfigure}{L}{2.3in}
%\begin{figure}
%\begin{center}
%\footnotesize
\small
%\normalsize
\vspace{5pt}
// \FI denotes  \prob{X}{F} \\
// \pnt{q} is an assignment to \V{F} \\
// \DS~denotes the current set of active \\
//~~~~~D-sequents \\
\vspace{-10pt}
\begin{tabbing}
aaaa\=bb\= c\= dddddddddddd\= \kill
\cdi\!\!(\FI,\pnt{q},\DS)\{\\
\tb{\scriptsize{1}}\> $\DS := \DS \cup \mi{AtomDseqs}(\Phi,\pnt{q},\DS)$ \\
\tb{\scriptsize{2}}\>if ($\mi{EveryXclauseRedund}(\Phi,\DS)$) \\
\tb{\scriptsize{3}}\Tt return($\Phi,\DS$)\\
\> - - - - - - - - - - - -  \\
\tb{\scriptsize{4}}\> $v := \mi{PickVar}(F,\pnt{q},\DS)$ \\
\tb{\scriptsize{5}}\> $(\Phi,\DS_0):=$\cdi\!\!(\FI,$\pnt{q}\cup\s{v=0}$,\DS)\\
\tb{\scriptsize{6}}\> $\DS := \mi{DropInapplic}(\DS_0,v)$ \\
\tb{\scriptsize{7}}\> $(\Phi,\DS_1):=$\cdi\!\!(\FI,$\pnt{q} \cup\s{v=1}$,\DS)\\
\tb{\scriptsize{8}}\> $\DS := \mi{JoinDseqs}(\Phi,v,\DS_0,\DS_1)$\\
\tb{\scriptsize{9}}\> return($\Phi,\DS$)\} \\
\end{tabbing} 
\vspace{-15pt}
\caption{\cdi procedure}
%\vspace{-10pt}
\label{fig:dcds}
%\end{figure}
\end{wrapfigure}



==> old_files/d6cds+.fig.tex <==
%
%
% DCDS+
%
\setlength{\intextsep}{2pt}
\setlength{\textfloatsep}{5pt}
\begin{wrapfigure}{l}{2.3in}
%\begin{figure}
%\begin{center}
%\footnotesize
\small
\vspace{5pt}
%\normalsize
// \FI denotes  \prob{X}{F} \\
// \pnt{q} is an assignment to \V{F} \\
// \DS~denotes the current set of active \\
//~~~~~D-sequents \\
// \PS denotes the set of stored D-sequents \\
\vspace{-10pt}
\begin{tabbing}
aaaa\=bb\= c\= dddddddddddd\= \kill
\Cdi\!\!(\FI,\pnt{q},\DS,\PS)\{\\
\tb{\scriptsize{1*}}\> $\DS := \DS \cup \mi{ReuseDseqs}(\FI,\pnt{q},\PS,\DS)$ \\
\tb{\scriptsize{2*}}\> $\DS := \DS \cup \mi{AtomDseqs}(\Phi,\pnt{q},\DS)$ \\
\tb{\scriptsize{3}}\>if ($\mi{EveryXclauseRedund}(\Phi,\DS)$) \\
\tb{\scriptsize{4}}\Tt return($\Phi,\DS,\PS$)\\
\> - - - - - - - - - - - -  \\
\tb{\scriptsize{5}}\> $v := \mi{PickVar}(F,\pnt{q},\DS)$ \\
\tb{\scriptsize{6}}\> $(\Phi,\DS_0,\PS):=$\Cdi\!\!($\Phi$,$\pnt{q}\cup\!(v=0)$,\DS,\PS)\\
\tb{\scriptsize{7}}\> $\DS := \mi{DropInapplic}(\DS_0,v)$ \\
\tb{\scriptsize{8}}\> $(\Phi,\DS_1,\PS):=$\Cdi\!\!($\Phi$,$\pnt{q}\cup\!(v=1)$,\DS,\PS)\\
\tb{\scriptsize{9*}}\> $\DS := \mi{JoinDseqs}^+(\Phi,v,\DS_0,\DS_1)$\\
\tb{\scriptsize{10*}}\> $\PS := \PS \cup DseqsToStore(\DS)$ \\
\tb{\scriptsize{11}}\> return($\Phi,\DS,\PS$)\} \\
\end{tabbing} 
\vspace{-15pt}
\caption{\Cdi procedure}
\vspace{5pt}
\label{fig:dcds+}
%\end{figure}
\end{wrapfigure}



==> old_files/d7cds+_alg.tex <==
\section{Introducing \Cdi}
\label{sec:dcds_plus}

In this section, we describe a modification of \cdi that re-uses
D-sequents. We will refer to it as \Cdi. The pseudocode of \Cdi is
shown in Fig.~\ref{fig:dcds+}. In comparison to \cdi, \Cdi has one
more input parameter: a set \PS of D-sequents stored to re-use. The
four lines where \Cdi behaves differently from \cdi are marked with an
asterisk.

%\input{d6cds+.fig}

The difference between \Cdi and \cdi is as follows.  First, \Cdi uses
the new definition of D-sequents and thus keeps track of order
constraints. (In particular, \Cdi stores order constraints when
generating the atomic D-sequents of the second/third kind.  For that
reason, line 2 is marked with an asterisk.) Second, \Cdi tries to
re-use D-sequents stored in \PS. Namely, if an $X$-clause $C$ is not
proved redundant yet, \Cdi checks if there is a D-sequent of \PS a)
that states redundancy of $C$; b) whose conditional \pnt{r} satisfies
$\pnt{r} \subseteq \pnt{q}$ and c) whose order constraint is
consistent with those of active D-sequents. Third, \Cdi stores some of
new D-sequents obtained by the join operation (line 10).

\input{j3oin_dseqs.fig}

The final difference between \Cdi and \cdi is as follows.  As we
mentioned in Subsection~\ref{ssec:dcds_corr}, merging results of the
two branches by the \jd procedure of \cdi may produce a set of
inconsistent D-sequents. If no D-sequents are re-used, as in \cdi,
this inconsistency does not mean that the D-sequents of this set are
not composable (see Subsection~\ref{ssec:dcds_corr}). However,
re-using D-sequents, as it is done in \Cdi, may produce inconsistent
D-sequents that are \ti{indeed} not composable. For that reason, in
\Cdi, a modification of \jd called \Jd is used.



The pseudocode of \Jd is shown in Fig.~\ref{fig:join_dseqs+}. The
objective of \Jd is to generate a set of \ti{consistent} D-sequents
that do not depend on variable $v$. The resulting D-sequents are
accumulated in \DS. \Jd starts by initializing \DS with the D-sequents
that are already symmetric in $v$ i.e. their conditionals do not
contain an assignment to variable $v$.  Then \Jd forms the set $G$ of
$X$-clauses whose D-sequents are asymmetric in $v$.



The main part of \Jd consists of a loop (lines 3-8) where, for every
clause $C$ of $G$, a D-sequent whose conditional is symmetric in $v$
is built. First, \Jd extracts D-sequents $S_0$ and $S_1$ of clause $C$
and joins them at variable $v$ to produce a D-sequent $S$ (lines
4-5). If the D-sequents of \DS become inconsistent after adding $S$,
\Jd calls $\mi{FixDseq}$ to produce a D-sequent $S$ that preserves the
consistency of \DS.  Proposition~\ref{prop:mak_rob} shows that it is
always possible.  Namely, one can always relax the order constraints
of $S_0$ and $S_1$ thus relaxing that of $S$.  In particular, one can
totally eliminate order constraints of $S_0$ and $S_1$, which makes
them (and hence $S$) robust.


==> old_files/f0ootnote.tex <==
A clause is a disjunction of literals. So a CNF formula $F$ is a
conjunction of clauses: $C_1 \wedge \dots \wedge Ck$. We will also
view $F$ just a set of clauses \s{C_1,\dots,C_k}. Given formula
\prob{X}{F} we will say that clause $C$ is redundant in \prob{X}{F} if
$\prob{X}{F} \equiv \prob{X}{F \setminus \s{C}}$.


==> old_files/f1ootnote.tex <==
Indeed, $\prob{X}{F^* \wedge F} \equiv \prob{X}{F}$ since $F
\rightarrow F^*$. On the other hand, $\prob{X}{F^* \wedge F} \equiv
\prob{X}{F^*} \equiv F^*$ since adding $F^*$ makes $F$ redundant and
$F^*$ does not depend on $X$.


==> old_files/f5ootnote.tex <==
For the sake of simplicity, Figure~\ref{fig:dcds} gives a very
abstract view of \cdi. For instance, we omit the lines of code where
new clauses are generated. Our objective here is just to show the part
of \cdi where D-sequents are involved. A more detailed description
of \cdi can be found in~\cite{fmcad13}.


==> old_files/f6ootnote.tex <==
In~\cite{hvc-14}, we introduced Partial QE (PQE) where only
a \ti{part} of the formula is taken out of the scope of
quantifiers. The appeal of PQE is twofold. First, many verification
problems like equivalence and model checking require partial rather
than complete QE~\cite{fmcad16,mc_no_inv}. Second, PQE is much simpler
to solve than QE. Both QE and PQE benefit from the results of this
paper. However, since QE is conceptually simpler than PQE, we picked
the former to introduce our new approach to D-sequent re-using.




==> old_files/f7ootnote.tex <==
An $X$-clause $C$ is said to be redundant in \prob{X}{F} if
$\prob{X}{F} \equiv \prob{X}{F \setminus \s{C}}$. In this paper, we
use the standard convention of viewing a set of clauses
\s{C_1,\dots,C_n} as an alternative way to specify the CNF formula
$C_1 \wedge \dots \wedge C_n$. So, the expression $H \setminus \s{C}$
denotes the CNF formula obtained from $H$ by removing clause $C$.



==> old_files/f8ootnote.tex <==
In~\cite{fmcad13}, we just give basic definitions. In~\cite{fmsd14},
we do provide a detailed theoretical consideration but it is meant for
D-sequents introduced in~\cite{fmcad12} expressing redundancy of
variables rather than clauses. 


==> old_files/f9ootnote.tex <==
We will introduce the notion of a consistent set of D-sequents later,
see Definition~\ref{def:cons_dseqs}. Consistency of D-sequents in
Proposition~\ref{prop:dseq_third_kind} means that $C_1,\dots,C_k$ are
redundant together in subspace
\pnt{q}=$\bigcup\limits_{i=1}^{i=k}\ppnt{q}{i}$. So clause $C$ is
blocked at variable $v$ in subspace \pnt{q}.


==> old_files/i1ntroduction.tex <==
\section{Introduction}
Many verification problems can be cast as an instance of the
Quantifier Elimination (QE) problem or its
variations\footnote{\input{f6ootnote}}. So any progress in solving the
QE problem is of great importance. In this paper, we consider the QE
problem for propositional CNF formulas with existential quantifiers.
Given formula \prob{X}{F(X,Y)} where $X$ and $Y$ are sets of
variables, the QE problem is to find a quantifier-free formula
$F^*(Y)$ such that $F^* \equiv
\prob{X}{F}$. In~\cite{fmcad12,fmcad13}, we introduced a new approach
to QE based on the following observation. Let us call a
clause\footnote{A clause is a disjunction of literals. So, a CNF
  formula is a conjunction of clauses.} of $F$ an \bm{X}\tb{-clause}
if it contains at least one variable of $X$. Solving the QE problem
\prob{X}{F(X,Y)} reduces to finding formula $F^*(Y)$ implied by $F$
that makes the $X$-clauses of $F$ \ti{redundant} in \prob{X}{F^*
  \wedge F} (and so $F^* \equiv \prob{X}{F}$ holds). 

To implement the approach above, we introduced an algorithm called
\cdi (Derivation of Clause D-Sequents). \cdi is based on the following
three ideas. First, \cdi branches on variables of $F$ to reach a
subspace where proving redundancy\footnote{\input{f7ootnote}} of
$X$-clauses (or making them redundant by adding a new clause) is
easy. Second, once an $X$-clause is proved redundant, \cdi stores this
fact in the form of a Dependency Sequent (\tb{D-sequent}). A D-sequent
is a record \oods{q}{C} where $C$ is an $X$-clause of $F$ and \pnt{q}
is an assignment to variables of $F$. This record states that $C$ is
redundant in \prob{X}{F} in subspace \pnt{q}. The third idea of \cdi
is to use a resolution-like operation called \ti{join} to merge the
results of branches. This join operation is applied to D-sequents
\oods{q'}{C} and \oods{q''}{C} derived in branches $v=0$ and $v=1$
where $v$ is a variable of $F$.  The result of this operation is a
D-sequent \oods{q}{C} where \pnt{q} does not contain variable $v$.

To make \cdi more efficient, it is natural to try to re-use a
D-sequent \oods{q}{C} in every subspace \pnt{r} where $\pnt{q}
\subseteq \pnt{r}$ (i.e. \pnt{r} contains all the assignments of
\pnt{q}). However, here one faces the following problem. Suppose that
\oods{q'}{C'} and \oods{q''}{C''} are two D-sequents where $\pnt{q'}
\subseteq \pnt{r}$ and $\pnt{q''} \subseteq \pnt{r}$. These D-sequents
are called \tb{composable} if individual redundancy of $C'$ and $C''$
also implies that they are redundant in \prob{X}{F}
\tb{together}\footnote{That is $\prob{X}{F} \equiv \prob{X}{H
    \setminus \s{C',C''}}$.}.  Here is a simple example of D-sequents
that are not composable. Let formula \prob{X}{F} contain two identical
$X$-clauses $C'$ and $C''$. Then D-sequents \ooods{\emptyset}{C'} and
\ooods{\emptyset}{C''} hold. They state that $C'$ and $C''$ are
redundant in \prob{X}{F} \ti{individually}. On the other hand, in
general, one cannot drop \ti{both} $C'$ and $C''$ from \prob{X}{F}.

\cdi cannot guarantee the composability of D-sequents. So, it does not
re-use them. The reason why D-sequents cannot be re-used as easily as,
say, conflict clauses in SAT-solvers~\cite{grasp,chaff} is as
follows. Redundancy of a clause in a formula is a \tb{structural}
property\footnote{This is true regardless of whether this formula has
  quantifiers.}. That is the fact that clause $C$ is redundant in
formula $F$ may not hold in a formula $F'$ logically equivalent to
$F$. On the other hand, re-using a conflict clause $C$ is based on the
fact that $C$ is implied by the initial formula $F$ and implication is
a \tb{semantic} property. That is $C$ is implied by \ti{every} formula
$F'$ logically equivalent to $F$.

In this paper, we address the problem of composability (and hence
re-usability) of D-sequents. Our approach is based on the following
observation. Consider the example above with two identical $X$-clauses
$C',C''$. The D-sequent \ooods{\emptyset}{C'} requires the presence of
clause $C'' \in F$. This means that $C''$ is supposed to be proved
redundant \ti{after} $C'$. On the contrary, the D-sequent
\ooods{\emptyset}{C''} requires the presence of $C' \in F$ and hence
$C'$ is supposed to be proved redundant after $C''$. So these two
D-sequents are not composable because they have conflicting orders of
proving redundancy of $C'$ and $C''$.

To fix the problem of order conflicts above, we extend the definition
of D-sequents given in~\cite{fmcad13} by adding an order constraint.
A new D-sequent is a record \ods{q}{H}{C} where $H$ is a subset of
$X$-clauses of \prob{X}{F}. The set $H$ is an order constraint saying
that the clauses of $H$ are supposed to be proved redundant \ti{after}
$C$. We show that if D-sequents are consistent (i.e. their order
constraints can be satisfied), then this set is composable. So, to
re-use a D-sequent in subspace \pnt{r}, one just needs to make sure
that this D-sequent is consistent with the D-sequents already applied
in this subspace.

The contribution of this paper is as follows. First, we give the
necessary definitions and propositions explaining the semantics of
D-sequents stating redundancy of
$X$-clauses\footnote{\input{f8ootnote.tex}}
(Sections~\ref{sec:basic},~\ref{sec:bnd_pnts},~\ref{sec:div_conq}
and~\ref{sec:virt_red}.)  Second, we give a new definition of
D-sequents facilitating their re-using (Section~\ref{sec:dseqs}).  We
also introduce the notion of consistent D-sequents and show that they
can be re-used.  Third, we re-visit definitions of atomic D-sequents
(i.e. D-sequents stating trivial cases of redundancy) and the join
operation to accommodate the D-sequents of the new kind
(Sections~\ref{sec:atom_dseqs} and~\ref{sec:join_dseqs}). Fourth, we
explain the problem of \cdi with D-sequent re-using in terms of the
theory developed in this paper (Sections~\ref{sec:reuse}
and~\ref{sec:dcds_recall}).  Fifth, we present \Cdi, a version of \cdi
that can safely re-use D-sequents (Section~\ref{sec:dcds_plus}).


==> old_files/j1oin_dseqs.tex <==
\section{Join Operation}
\label{sec:join_dseqs}
In this section, we describe the operation of joining D-sequents that
produces a new D-sequent from two parent D-sequents. In contrast
to~\cite{fmcad13}, the join operation introduced here is applied to
D-sequents \ti{with order constraints}.



%
% Resolution of  assignments
%
\begin{definition}
\label{def:res_part_assgns}
Let \pnt{q'} and \pnt{q''} be assignments in which exactly one
variable $v \in \Va{q'} \cap \Va{q''}$ is assigned different values.
The assignment \pnt{q} consisting of all the value assignments of
\pnt{q'} and \pnt{q''} but those to $v$ is called the \tb{resolvent}
of \pnt{q'},\pnt{q''} on $v$.  Assignments \pnt{q'},\pnt{q''} are
called \tb{resolvable} on $v$.
\end{definition}
%
%  The join rule of DS-calculus
%
\begin{proposition}
\label{prop:join_rule}
Let \prob{X}{F} be an \ecnf formula for which D-sequents
\nods{q'}{H'}{C} and \ods{q''}{H''}{C} hold. Let \pnt{q'}, \pnt{q''}
be resolvable on $v \in \V{F}$ and \pnt{q} be the resolvent of
\pnt{q'} and \pnt{q''}.  Let $H = H' \cup H''$.  Then the D-sequent
\ods{q}{H}{C} holds.
\end{proposition}

%
% Joining D-sequents
%
\begin{definition}
\label{def:join_rule}
We will say that the D-sequent \ods{q}{H}{C} of
Proposition~\ref{prop:join_rule} is produced by \tb{joining
  D-sequents} \ods{q'}{H'}{C} and \ods{q''}{H''}{C} \tb{at} \bm{v}.
%We will call this D-sequent  the \tb{resolvent} of these two D-sequents on  $v$.
\end{definition}
%
% Remark about a stronger order constraint
%
\begin{remark}
  \label{rem:ord_constr}
  Note that the D-sequent $S$ produced by the join operation has a
  \ti{stronger} order constraint than its parent D-sequents. The
  latter have order constraints $H'$ and $H''$ in subspaces $v=0$ and
  $v=1$, whereas $S$ has the same order constraint $H = H' \cup H''$
  in either subspace. Due to this ``imprecision'' of the join
  operation, a set of D-sequents with conflicting order constraints
  can still be correct (see Section~\ref{sec:reuse} and
  Subsection~\ref{ssec:dcds_corr}).
\end{remark}


==> old_files/j2oin_dseqs_proofs.tex <==
\section*{Propositions of Section~\ref{sec:join_dseqs}: Join Operation}

%
%  Proposition: join operation
%
\begin{proposition}
%\label{prop:join_rule}
  Let \,\prob{X}{F} be an \ecnf formula. Let D-sequents \ods{q'}{H'}{C}
and \ods{q''}{H''}{C} hold. Let \pnt{q'}, \pnt{q''} be resolvable on
$v \in \V{F}$ and \pnt{q} be the resolvent of \pnt{q'} and \pnt{q''}.
Let $H = H' \cup H''$.  Then the D-sequent \ods{q}{H}{C} holds.
\end{proposition}
%
%
%
\begin{mmproof}
Denote by $S'$ and $S$ the D-sequents \ods{q'}{H'}{C} and
\ods{q}{H}{C} respectively. Assume that $S$ does not hold. Then there
is a member formula $W$ of $S$ such that $C$ is not redundant in
\prob{X}{\cof{W}{q}} even virtually.  This means that
%
\begin{itemize}
\item the set $B$ of Definition~\ref{def:virt_red} is not empty and
\item there is a point $\pnt{p} \in B$ that is $X$-removable in every
  formula \cof{W}{r} where $\pnt{q^*} \subseteq \pnt{r} \subset
  \pnt{q}$ (see Definition~\ref{def:virt_red}).
\end{itemize}
 Assume for the sake of clarity that \pnt{p} has the same assignment
 to $v$ as \pnt{q'}. Note that, since $H' \subseteq H$, $W$ is a
 member formula of the D-sequent \ods{q'}{H'}{C}. So, \cof{C}{q'} is
 redundant in \prob{X}{\cof{W}{q'}}.  Consider the following
 possibilities.
 \begin{itemize}
   %
 \item Point \pnt{p} \,is not $X$-removable in \cof{W}{q'} and $v \in
   X$. Then it is not $X$-removable in \cof{W}{s} where \pnt{s} is
   obtained from \pnt{q'} by dropping the assignment to $v$. Since
   $\pnt{s} \subset \pnt{q}$ \,holds, this contradicts the fact that
   \pnt{p} has to be $X$-removable in every subspace $\pnt{q^*}
   \subseteq \pnt{r} \subset \pnt{q}$.
   %
 \item Point \pnt{p} \,is not $X$-removable in \cof{W}{q'} and $v
   \not\in X$.  Then \pnt{p} \,is not $X$-removable in \cof{W}{q}.
   This contradicts the fact that $\pnt{p} \in B$.
  %
   \item Point \pnt{p} \,is $X$-removable in \cof{W}{q'} and it is
     $X$-removable in \cof{W}{r} for every $\vec{q'}^* \subseteq
     \pnt{r} \subset \pnt{q'}$.  Then \cof{C}{q'} is not redundant in
     \prob{X}{\cof{W}{q'}}, \vspace{3pt} which contradicts the fact
     that D-sequent $S'$ holds.
   %
 \item Point \pnt{p} is $X$-removable in \cof{W}{q'}, and $v \in X$
   and \pnt{p} is not $X$-removable in \cof{W}{r} where $\vec{q'}^*
   \subseteq \pnt{r} \subset \pnt{q'}$.  Then it is not $X$-removable
   in \cof{W}{r^*} obtained from \pnt{r} by dropping the assignment to
   $v$, if any (regardless of whether or not $v$ is in $X$).  Since
   $\pnt{r^*} \subset \pnt{q}$ holds, this contradicts the fact that
   \pnt{p} \,has to be $X$-removable in every subspace $\pnt{q^*}
   \subseteq \pnt{r} \subset \pnt{q}$.  $\square$
 \end{itemize}

\end{mmproof}


==> old_files/j3oin_dseqs.fig.tex <==
%
% merge procedure
%
\setlength{\intextsep}{4pt}
\setlength{\textfloatsep}{10pt}
\begin{wrapfigure}{l}{2in}
%\begin{figure}
%\begin{center}
\small
%\normalsize
%\vspace{5pt}
\begin{tabbing}
aaa\=bb\= cc\= ddddddd\= \kill
$\mi{JoinDseqs}^+(\Phi,v,\DS_0,\DS_1)$\{\\
\tb{\scriptsize{1}}\> $\DS := \mi{SymmDseqs}(\DS_0)$ \\
\tb{\scriptsize{2}}\> $G := \mi{FormXcls}(\DS_0 \setminus \DS)$ \\
\tb{\scriptsize{3}}\> foreach ($C \in G$) \{ \\
\tb{\scriptsize{4}}\Tt  $(S_0,S_1) := \mi{ExtrDseqs}(\DS_0,\DS_1,C)$\\
\tb{\scriptsize{5}}\Tt  $S := \mi{join}(S_0,S_1,v)$ \\
\tb{\scriptsize{6}}\Tt  if ($\mi{incons}(\DS \cup \s{S})$) \\
\tb{\scriptsize{7}}\ttt   $S := \mi{FixDseq}(S,\DS,\DS_0,\DS_1)$ \\
\tb{\scriptsize{8}}\Tt  $\DS := \DS \cup \s{S}$ \}\\
\tb{\scriptsize{9}}\> return(\DS);\} \\
\end{tabbing} 
\vspace{-20pt}
\caption{$\mi{JoinDseqs}^+$ procedure}
\label{fig:join_dseqs+}
%\end{figure}
\end{wrapfigure}


==> old_files/proofs.tex <==
%\clearpage
\appendix
\setcounter{proposition}{0}
\vspace{10pt}
\noindent\tb{\large{Appendix}} \\
\vspace{10pt}

The appendix contains proofs of the propositions listed in the paper.
We also give proofs of lemmas used in the proofs of propositions.

\input{b2nd_pnts_proofs}
\input{d1iv_conq_proofs}
\input{v1irt_redund_proofs}
%\input{s3imple_cases_proofs}
%\input{d3ep_sequents_proofs}
\input{a3tomic_dseqs_proofs}
\input{j2oin_dseqs_proofs}
\input{r3euse_dseqs_proofs}
\input{t1ransform_dseqs_proofs}



==> old_files/r2euse_dseqs.tex <==
\section{Re-usability of D-sequents}
\label{sec:reuse}
To address the problem of D-sequent re-using, we introduce the notion
of composability. Informally, a set of D-sequents is composable if the
clauses stated redundant individually are also redundant
\ti{collectively}.  Robust D-sequents are always composable. So they
can be re-used in any context like conflict clauses in
SAT-solvers. However, this is not true for fragile D-sequents. Below,
we show that such D-sequents are composable if they are consistent.
So it is safe to re-use a fragile D-sequent in a subspace \pnt{q}, if
it is consistent with the D-sequents already used in subspace \pnt{q}.

% 
% Definition: compatible assignments
%
\begin{definition}
  Assignments \pnt{q'} and \pnt{q''} are called \tb{compatible} if
  every variable from $\Va{q'} \cap \Va{q''}$ is assigned the same
  value.
\end{definition}

%
% Definition: composable D-sequents
%
\begin{definition}
\label{def:comp_dseqs}
  Let \,\prob{X}{F} be an \,\ecnf.  A set of D-sequents
  \oDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$, \oDs{\ppnt{q}{k}}{H_k}{C_k} is
  called \tb{composable} if the clauses \s{C_1,\dots,C_k} are
  redundant collectively as well. That is $\prob{X}{F} \equiv$
  \Prob{X}{F \setminus \s{C_1,\dots,C_k}} holds in subspace \pnt{q}
  where \pnt{q}=$\bigcup\limits_{i=1}^{i=k}\ppnt{q}{i}$.
\end{definition}


%
% Definition: Consistent D-sequents
%
\begin{definition}
\label{def:cons_dseqs}
  Let \prob{X}{F} be an \ecnf. A set of D-sequents
  \oDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$, \oDs{\ppnt{q}{k}}{H_k}{C_k} is
  called \tb{consistent} if
  \begin{itemize}
  \item every pair of assignments \pnt{q_i},\pnt{q_j}, $1 \leq i,j \leq k$
    is compatible;
  \item there is a total order $\pi$ over clauses of
    $\bigcup\limits_{i=1}^{i=k} H_i \cup \s{C_i}$ that \vspace{4pt}
    satisfies the order constraints of these D-sequents
    i.e. $\forall{C} \in H_i$, $\pi(C_i) < \pi(C)$ holds where
    $i=1,\dots,k$.
  \end{itemize} 
\end{definition}

%
% Proposition: consistent set of D-seqs.
%
\begin{proposition}
\label{prop:cons_dseqs}
 Let \prob{X}{F} be an \ecnf. Let \oDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$,
 $(\ppnt{q}{k},H_k)$ $\rightarrow C_k$ be a consistent set of
 D-sequents. Then these D-sequents are composable and hence clauses
 \s{C_1,\dots,C_k} are collectively redundant in \prob{X}{F} in
 subspace \pnt{q} where \pnt{q}=$\bigcup\limits_{i=1}^{i=k}
 \ppnt{q}{i}$.
\end{proposition}
%
%  Example: inconsistency does not mean that incomposability
%
\begin{remark}
  The fact that D-sequents $S_1,\dots,S_k$ are inconsistent does not
  necessarily mean that these D-sequents are not composable.  As we
  mentioned in Remark~\ref{rem:ord_constr}, as far as order
  constraints are concerned, the join operation is not ``precise''.
  This means that if the D-sequents above are obtained by applying the
  join operation, their order-inconsistency may be artificial. An
  example of that is the QE procedure called \cdi~\cite{fmcad13}. As
  we explain in Subsection~\ref{ssec:dcds_corr}, if one uses the new
  definition of D-sequents (i.e.  Definition~\ref{def:dseq}), the
  D-sequents produced by \cdi are, in general, inconsistent.  However,
  \cdi is provably correct~\cite{fmsd14}.
\end{remark}
%
% Remark: Solving QE
%
\begin{remark}
  Let \prob{X}{F(X,Y)} be an \ecnf and $R(X,Y)$ be the set of clauses
  added to $F$ by a QE-solver. Let $F^X \cup R^X =\s{C_1,\dots,C_k}$
  (i.e. the latter is the set of all $X$-clauses of $F \cup R$).  This
  QE-solver terminates when the set\footnote{This set consists of the
    clauses of $R$ that depend \ti{only} on variables of $Y$.} $R
  \setminus R^X$ is sufficient to derive consistent D-sequents
  $(\prob{X}{F \wedge R}$,$\emptyset,H_1)$ $\rightarrow C_1$, $\dots$,
  $(\prob{X}{F \wedge R}$,$\emptyset,H_k)$ $\rightarrow C_k$. From
  Proposition~\ref{prop:cons_dseqs} it follows, that all $X$-clauses
  can be dropped from \prob{X}{F \wedge R}. The resulting formula
  $F^*(Y)$ consisting of clauses of $F \cup R \setminus
  \s{C_1,\dots,C_k}$ is logically equivalent to \prob{X}{F}.
\end{remark}





==> old_files/r3euse_dseqs_proofs.tex <==
\section*{Propositions of Section~\ref{sec:reuse}: Re-usability of D-sequents}
%

%
% Proposition: A consistent set of D-sequents.
%
\begin{proposition}
%\label{prop:cons_dseqs}
Let \prob{X}{F} be an \ecnf. Let \oDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$,
$(\ppnt{q}{k},H_k)$ $\rightarrow C_k$ be a consistent set of
D-sequents. Then these D-sequents are composable and hence clauses
\s{C_1,\dots,C_k} are collectively redundant in \prob{X}{F} in
subspace \pnt{q} where \pnt{q}=$\bigcup\limits_{i=1}^{i=k}
\ppnt{q}{i}$.
\end{proposition}
%
\begin{mmproof}
Since $\ppnt{q}{i} \subseteq \pnt{q}$, $i=1,\dots,k$, from
Proposition~\ref{prop:subspace} it follows that D-sequents
\ods{q}{H_i}{C_i}, $i=1,\dots,k$ hold. Assume for the sake of
simplicity that $\pi(C_i) < \pi(C_j)$ if $i < j$. Then one can prove
redundancy of clauses $C_i$, $i=1,..,k$ in subspace \pnt{q} \,in the
order they are numbered. Denote \ods{q}{H_i}{C_i} as $S_i$,
$i=1,\dots,k$.  Denote by $F_{i+1}$ formula $F \setminus
\s{C_1,\dots,C_i}$, $i=1,\dots,k$. Formula $F_1$ is set to $F$.  Since
$S_1$ is applicable to $F_1$ one can remove $C_1$ in subspace \pnt{q}
producing formula $F_2$.  Note that $F_2$ is a member formula for
$S_2$. By applying $S_2$ to $F_1$ one removes clause $C_2$ in subspace
\pnt{q} producing $F_3$, a member formula for $S_3$. Going on in such
a manner one eventually produces formula $F_{k+1}$ thus showing that
\s{C_1,\dots,C_k} are redundant in \prob{X}{F} in subspace
\pnt{q}. $\square$
\end{mmproof}



==> old_files/s0ources.tex <==
\begin{proposition}
  \label{prop:uns_cls}
 Let \prob{X}{F} be an \ecnf formula and \pnt{q} be an assignment
  to \V{F}.  Let $B,C$ be two clauses of $F$. Let \cof{C}{q} be an
  $X$-clause and \cof{B}{q} imply \cof{C}{q} (i.e. every literal of
  \cof{B}{q} is in \cof{C}{q}). Then the D-sequent \ods{q}{H}{C} holds
  where $H = \s{B}$ if \cof{B}{q} is an $X$-clause and $H = \emptyset$
  otherwise.  We will refer to the D-sequent above as an atomic
  D-sequent of the \tb{second kind}.
\end{proposition}
--------
% SUBSECTION: Definition of D-sequents
%
\subsection{Definition of D-sequents}
\label{ssec:def_dseqs}
---------
In Subsection~\ref{ssec:frag_rob}, we use this new
definition to discuss robustness/fragility of D-sequents.
------
%
% Subsection: Fragile and robust D-sequents
%
\subsection{Fragile and robust D-sequents}
\label{ssec:frag_rob}
Suppose that a QE algorithm currently explores branch \pnt{r}. Let
$S'$ denote D-sequent \oods{q}{C'} (with an empty order constraint)
and $S''$ denote D-sequent \ods{q}{H}{C''} where $C' \in H$. Suppose
that $S'$ and $S''$ have been derived in a branch different from
\pnt{r}.  Assume that $\pnt{q} \subseteq \pnt{r}$ and consider
re-using $S'$ and $S''$ in subspace \pnt{r}. Suppose that first we use
$S'$ to claim redundancy of clause $C'$. Note that this violates the
order constraint of D-sequent $S''$ and hence invalidates it.


Since a D-sequent with non-empty order constraint can be invalidated
by some other D-sequent used earlier, we will call the former
\tb{fragile}. ($S''$ is an example of a fragile D-sequent.) Otherwise,
we will call a D-sequent \tb{robust}.  D-sequent $S'$ is an example of
a robust D-sequent. Application of a robust D-sequent is not affected
by other D-sequents.  For instance, D-sequent $S'$ is still valid
after applying D-sequent $S''$.
--------
%
%  D-sequent
%
\begin{definition}
\label{def:dseq}
Let \prob{X}{F} be an \ecnf formula. Let \pnt{q} be an assignment to
\V{F} and $H \subseteq F^X$ and $C \in F^X$ where $C \not\in H$.  A
dependency sequent (\tb{D-sequent}) $S$ has the form
\Ods{X}{F}{q}{H}{C}. It states that clause \cof{C}{q} is redundant in
every formula \prob{X}{\cof{W}{q}} logically equivalent to
\prob{X}{\cof{F}{q}} where
\begin{itemize}
\item $H \cup \s{C} \subseteq W \subseteq F$ and
\item every clause of $F \setminus W$ (if any) is an $X$-clause in
  subspace \pnt{q}.
\end{itemize}
\pnt{q} and $H$ are called the \tb{conditional} and \tb{order
  constraint} of $S$ respectively. We will refer to $W$ as a
\tb{member formula} for $S$.
\end{definition}
----------
\begin{mmproof}
Since $\ppnt{q}{i} \subseteq \pnt{q}$, $i=1,\dots,k$, from
Proposition~\ref{prop:subspace} it follows that D-sequents
\ods{q}{H_i}{C_i}, $i=1,\dots,k$ hold. Assume for the sake of
simplicity that $\pi(C_i) < \pi(C_j)$ if $i < j$. Then one can prove
redundancy of clauses $C_i$, $i=1,..,k$ in subspace \pnt{q} \,in the
order they are numbered. The fact that $\pi$ satisfies the order
constraints guarantees that after proving redundancy of
$C_1,\dots,C_i$ one can still apply D-sequent
\oDs{\pnt{q}}{H_{i+1}}{C_{i+1}} to claim redundancy of $C_{i+1}$ in
subspace \pnt{q}.~$\square$
\end{mmproof}
----
\begin{mmproof}
  Assume that \V{F} are assigned as in \pnt{q'} and clauses of $H'
  \setminus \s{C''}$ are not proved redundant yet. Let us show that
  $C'$ is redundant in \prob{X}{F} in subspace \pnt{q'} and so
  \ods{q'}{H' \setminus \s{C''}}{C'} holds. Consider the following two
  situations.  First, assume that clause $C''$ is not proved redundant
  yet. Then the D-sequent \ods{q'}{H'}{C'} holds and so $C'$ is
  redundant in \prob{X}{F} in subspace \pnt{q'}.

  Now assume that clause $C''$ is \ti{already proved} redundant.
  Denote D-sequents \ods{q'}{H'}{C'} and \ods{q''}{H''}{C''} by $S'$
  and $S''$ respectively. Denote by $S^{*}{''}$ the D-sequent used to
  prove redundancy of $C''$. Let $S^{*}{''},Q_1,\dots,Q_p$ specify the
  order in which $S^{*}{''}$ and the following D-sequents are
  applied. Below, we show that one can transform this sequence of
  valid D-sequents into the sequence $Q_1,\dots,Q_p,S',S''$. Every
  D-sequent of the new sequence is valid in its position including
  D-sequent $S'$ proving redundancy of clause $C'$.

  First, note that one can replace $S^{*}{''}$ with $S''$ in the
  original sequence since clauses of $H' \setminus {C'}$ are not
  proved redundant yet and $H'' \subset H'$ holds. For the same
  reason, one can replace sequence $S'',Q_1,\dots,Q_p$ with
  $Q_1,\dots,Q_p,S''$. Indeed, pushing $S''$ forward cannot make a
  D-sequent $Q_i$ invalid $i=1,\dots,p$. Besides, $S''$ is valid even
  after applying D-sequents $Q_1,\dots,Q_n$. Finally, one can insert
  D-sequent $S'$ before $S''$ to produce sequence
  $Q_1,\dots,Q_p,S',S''$. Indeed, $S'$ is still valid after applying
  $Q_1,\dots,Q_n$ and does not invalidate $S''$ (because $H''$ does
  not contain $C'$).
\end{mmproof}
-----
%
% Lemma: sat. assign for cofactor
%
\begin{lemma}
Let $F$ be a CNF formula. Let \pnt{q} be an assignment to \V{F}. Let
\pnt{p} be an assignment satisfying \cof{F}{q} such that $\pnt{q}
\subseteq \pnt{p}$. Then \pnt{p} satisfies $F$ as well.
\end{lemma}
%
%
%
\begin{lemma}
  Let \prob{X}{F(X,Y)} be an \ecnf formula. Let $C$ be an $X$-clause
  that is (virtually) redundant in \prob{X}{F} in subspace
  \pnt{q}. Then every point that falsifies only clause \cof{C}{q} in
  \cof{F}{q} can be turned into an assignment satisfying $F$ by
  changing a subset of variables of $X$.
\end{lemma}
--------
\begin{mmproof}
From Lemma~\ref{lem:red_add_cls} it follows\footnote{For the sake of
  simplicity, we proved Lemma~\ref{lem:red_add_cls} in terms of global
  rather than local redundancy of $C$ i.e. redundancy in \prob{X}{F}
  rather than in \prob{X}{\cof{F}{q}}. This lemma can be easily
  reformulated and proved in terms of local redundancy.} that clause
$C$ is redundant in \prob{X}{F \wedge R} in subspace \pnt{q}. The
order constraint $H$ is not affected by adding $R$ to $F$.
\end{mmproof}
-------
%
%  Lemma: Red still holds after adding implications
%
\begin{lemma}
\label{lem:red_add_cls}
Let $X$-clause $C$ be redundant in \prob{X}{F}. Let $R$ be a CNF
formula implied by $F$. Then $C$ is redundant in \prob{X}{F \wedge R}
as well.
\end{lemma}
%
% proof
%
\begin{mmproof}
Denote $F \wedge R$ as $F'$.  Assume the contrary, \ie $C$ is
redundant in \prob{X}{F} but not in \prob{X}{F'}.  The latter means
that there is a boundary point \pnt{p} of $F'$ such that \pnt{p}
falsifies only clause $C$ and \pnt{p} \,is $X$-removable in $F'$.

Since $C$ is in $F$, \pnt{p} \,is a boundary point of $F$ as well. Let
us show that \pnt{p} \,is also $X$-removable in $F$, which means that
$C$ is not redundant in \prob{X}{F} and we have a contradiction.
Assume the contrary, i.e. \pnt{p} \,is not $X$-removable in $F$. Then
there is a point \pnt{s} satisfying $F$ obtained from \pnt{p} by
flipping values of variables of $X$. Since $F \Rightarrow R$ holds,
\pnt{s} satisfies $R$ too and hence it satisfies $F'$. This
contradicts the fact that \pnt{p} is $X$-removable in $F'$.  $\square$
\end{mmproof}
-------
\begin{mmproof}
  Assume that the clauses of $H \cup G$ are not proved redundant yet.
  Then the order constraint of D-sequent \ods{q}{H}{C} is satisfied
  and \cof{C}{q} is redundant in \prob{X}{\cof{F}{q}}. Hence,
  \ods{q}{H \cup G}{C} holds too.
\end{mmproof}

\begin{mmproof}
Since \cof{C}{q} is blocked in \cof{F}{q} with respect to variable
$v$, \cof{C}{q} is redundant in \prob{X}{\cof{F}{q}} (see
Lemma~\ref{lem:blk_cls}). This redundancy does not require the
presence of any clauses in \cof{F}{q} (other than \cof{C}{q}
itself). So, no order constraint is necessary and D-sequent
\oods{q}{C} holds. $\square$
\end{mmproof}
----------
%
%  Example
%
\begin{example}
  Let \prob{X}{F(X,Y)} be an \ecnf. Let $C_3,C_6,C_8$ be the only
  clauses of $F$ with variable $x_5 \in X$ where $C_3 = x_5 \wedge
  x_{10} $, $C_6 = \overline{x}_5 \wedge y_1$, $C_8 = \overline{x_5}
  \vee y_3 \vee y_5$. Note that assignment $y_1=1$ satisfies clause
  $C_6$.  So the D-sequent \ooods{(y_1=1)}{C_6} holds. Suppose that a
  D-sequent \oods{r}{C_8} holds as well where $\pnt{r} =
  (y_2=0,x_{10}=1)$. Since, these D-sequents hold in subspace $\pnt{q}
  = (y_1=1,y_2=0,x_{10}=1)$, clause $C_3$ is blocked with respect to
  variable $x_5$ in subspace \pnt{q}. From
  Proposition~\ref{prop:dseq_third_kind} it follows that the D-sequent
  \oods{q}{C_3} holds.
\end{example}

\begin{proposition}
  \label{prop:dseq_third_kind}
Let \prob{X}{F} be an \ecnf. Let $C$ be an $X$-clause of $F$ and $v
\in\V{C} \cap X$. Let $C_1,\dots,C_k$ be the clauses of $F$ that can
be resolved with $C$ on variable $v$. Let \pnt{q} specify a subspace
where the clauses $C_1,\dots,C_k$ are redundant. (That is \cof{C}{q}
is blocked in \cof{F}{q} with respect to $v$.) Then D-sequent
\oods{q}{C} holds. We will refer to it as an atomic D-sequent of the
\tb{third kind}.
\end{proposition}
-------
\begin{mmproof}
Let $W$ be a formula of Definition~\ref{def:dseq}. That is
$\prob{X}{\cof{W}{q}} \equiv \prob{X}{\cof{F}{q}}$ and $\s{C}
\subseteq W \subseteq F$.  Since \cof{B}{q} implies \cof{C}{q}, then
$\cof{F}{q} \equiv \cof{F}{q} \setminus \s{\cof{C}{q}}$.$\square$
\end{mmproof}

----------
\,\footnote{Note that the clause \cof{C}{q} equal to \ti{true}
  remains in \cof{H}{q} rather than being removed from \cof{H}{q}.  We
  treat such a clause as \ti{redundant} in \cof{H}{q} (see
  Proposition~\ref{prop:sat_cls}).}
-----------  
It states that clause \cof{C}{q} is redundant in
every formula \prob{X}{\cof{W}{q}} that is logically equivalent to
\prob{X}{\cof{F}{q}} where $H \cup \s{C} \subseteq W \subseteq F$.
-----------
\begin{mmproof}
Since \cof{B}{q} implies \cof{C}{q}, then $\cof{F}{q} \equiv
\cof{F}{q} \setminus \s{\cof{C}{q}}$. The redundancy of \cof{C}{q}
depends on the presence of clause \cof{B}{q} in \cof{F}{q}. So if
\cof{B}{q} is an $X$-clause, its redundancy is supposed to be proved
after that of \cof{C}{q}. Hence one needs an order constraint.$\square$
\end{mmproof}
-----------
\begin{mmproof}
  Let \pnt{q} denote $(v=b)$. Clause \cof{C}{q} is \ti{true} and so is
  redundant in \cof{F}{q}. No presence of clauses is required to
  guarantee the redundancy of \cof{C}{q}. So, no order constraint is
  necessary and the D-sequent \ooods{(v=b)}{C} holds. $\square$
\end{mmproof}
----
\begin{definition}
\label{def:dseq}
Let \prob{X}{F} be an \ecnf formula. Let \pnt{q} be an assignment to
\V{F} and $H \subseteq F^X$ and $C \in F^X$ where $C \not\in H$.  A
dependency sequent (\tb{D-sequent}) $S$ has the form
\Ods{X}{F}{q}{H}{C}. It states that clause \cof{C}{q} is redundant in
\prob{X}{\cof{F}{q}} under an \tb{order constraint} specified by $H$.
We will call \pnt{q} the \tb{conditional} of the D-sequent $S$.  The
order constraint $H$ says that $S$ can be used \tb{only} if no clause
of \cof{H}{q} is proved redundant in \prob{X}{\cof{F}{q}} yet. In
other words, the redundancy of clauses of \cof{H}{q} must be proved
\tb{after} that of clause \cof{C}{q}.
\end{definition}

Adding an order constraint differentiates Definition~\ref{def:dseq}
from that of~\cite{fmcad13}. The introduction of order constraints
enables checking if D-sequents are composable, thus making D-sequent
re-using possible (see Subsection~\ref{sec:reuse} and
Section~\ref{sec:dcds_plus}).
----------
(For the sake of simplicity, we
assume here that given an $X$-clause, its D-sequents in $\DS_0,\DS_1$
are either both symmetric or both asymmetric in $v$.)
--------
(That is the clauses
specified by the D-sequents of this set are redundant individually but
not collectively.)
---------
The D-sequents of $\DS_0$ and $\DS_1$ containing
assignment $v=0$ and $v=1$ respectively are joined at variable
$v$. Then \cdi terminates returning \prob{X}{F} and the D-sequents
obtained by merging branches $v=0$ and $v=1$.
---------
In this section, we describe two transformations of D-sequents used by
\Cdi, a modification of procedure \cdi of~\cite{fmcad13} introduced in
this paper (see Section~\ref{sec:dcds_plus}).  Similarly to \cdi, \Cdi
adds new clauses to make $X$-clauses redundant. So, in general,
D-sequents of different branches are computed with respect to
different formulas.  In Subsection~\ref{ssec:align}, we describe a
transformation meant for ``aligning'' such D-sequents. \Cdi maintains
the following invariant: the D-sequents produced when merging results
of different branches by the join operation are consistent. Sometimes,
this requires relaxing order constraints of parent D-sequents to make
the latter more robust.  In Subsection~\ref{ssec:mak_rob}, we describe
a transformation meant for achieving this goal.
----------
Let \prob{X}{F(X,Y)} be an \ecnf and $F^X =\s{C_1,\dots,C_k}$
(i.e. the latter is the set of all $X$-clauses of $F$).  QE comes down
to finding a formula $R(Y)$ implied by $F$ for which there exists a
consistent set of D-sequents $(\prob{X}{F \wedge R}$,$\emptyset,H_1)$
$\rightarrow C_1$, $\dots$, $(\prob{X}{F \wedge R}$,$\emptyset,H_k)$
$\rightarrow C_k$. From Proposition~\ref{prop:cons_dseqs} it follows,
that all $X$-clauses of $F$ can be dropped from \prob{X}{F \wedge
  R}. The resulting formula $F^*$ (consisting of clauses of $F \cup R
\setminus \s{C_1,\dots,C_k}$) is logically equivalent to \prob{X}{F}.
--------
To address the problem of D-sequent re-using, in
Subsection~\ref{ssec:comp_dseqs}, we introduce the notion of
composability. Informally, a set of D-sequents is composable if the
clauses stated redundant individually are also redundant
\ti{collectively}.  Robust D-sequents are always composable. So they
can be re-used in any context like conflict clauses in
SAT-solvers. However, this is not true for fragile D-sequents. In
Subsection~\ref{ssec:cons_dseqs}, we show that such D-sequents are
composable if they are consistent.  So it is safe to re-use a fragile
D-sequent in a subspace \pnt{q}, if it is consistent with the
D-sequents already used in subspace \pnt{q}.
---------
%
% Consistent D-sequents
%
\subsection{Consistent D-sequents}
\label{ssec:cons_dseqs}
------
%
% Subsection
%
\subsection{Composable D-sequents}
\label{ssec:comp_dseqs}
-------
For the sake of simplicity, Proposition~\ref{prop:elim_incr} below is
presented in terms of global rather than local redundancy in subspace
\pnt{q} (i.e. redundancy in formula \prob{X}{F} rather than
\prob{X}{\cof{F}{q}}).
-------
\begin{definition}
 \label{def:X_clause}
 A clause $C$ of $F(X,Y)$ is called an \bm{X}\tb{-clause} if \V{C}
 $\cap~X~\neq~\emptyset$. Denote by \bm{F^X} the set of all
 $X$-clauses of $F$.
\end{definition}
------
Let \pnt{q} be an assignment, $F$ be a CNF formula, and $C$ be a
clause. \bm{\Va{q}} denotes the variables assigned in \pnt{q};
\bm{\V{F}} denotes the set of variables of $F$; \bm{\V{\prob{X}{F}}}
denotes $\V{F} \setminus X$; \bm{\V{C}} denotes the variables of $C$.
-------
Proposition~\ref{prop:dseq_add_cls} is very useful in ``aligning'' a
set of D-sequents. Suppose, for instance, that \ODs{X}{F \wedge
  R_1}{\ppnt{q}{1}}{H_1}{C_1},...,\ODs{X}{F \wedge
  R_k}{\ppnt{q}{k}}{H_1}{C_k}, where $F \rightarrow R_i,i=1,\dots k$,
satisfy the two conditions of Definition~\ref{def:cons_dseqs} for a
consistent set of D-sequents.  Note that these D-sequents do not
satisfy the entire definition because they are computed with respect
to different formulas \prob{X}{F \wedge R_i}, $i=1,\dots,k$.  Using
Proposition~\ref{prop:dseq_add_cls}, one can produce a new set of
D-sequents \ODs{X}{F \wedge R}{\ppnt{q}{1}}{H_1}{C_1},...,\ODs{X}{F
  \wedge R}{\ppnt{q}{k}}{H_1}{C_k} where $R = R_1 \wedge \dots \wedge
R_k$ that \ti{does} satisfy Definition~\ref{def:cons_dseqs}.
--------
Below, we
explain why the inconsistency of D-sequents produced by \jd does not
affect the correctness of \cdi.
--------
The fact that a set of D-sequents is inconsistent does not necessarily
mean that these D-sequents are not composable. This inconsistency can
be simply caused by the ``imprecision'' of the join
operation. Suppose, for instance, that one joins D-sequents $S'$ and
$S''$ at variable $v$ producing a D-sequent $S$.  Let $H'$ and $H''$
be the order constraints of $S'$ and $S''$. Then the order constraint
of $S$ is $H' \cup H''$. Note that D-sequent $S$ is ignorant of the
fact that order constraints $H'$ and $H''$ were used in subspaces
$v=0$ and $v=1$.  Instead, it assumes that, in either branch, one used
the same order constraint $H$ that is \ti{stronger} than $H'$ and
$H''$. So the inconsistency of D-sequents produced by \jd of \cdi is
just a side effect of imprecision of the join operation.
------------
%
% Lemma: subsitutution
%
\begin{lemma}
  \label{lem:subst}
  Let \prob{X}{F} be an \ecnf. Let D-sequents
  \oDs{\ppnt{q}{1}}{H_1}{C_1} and $(\ppnt{q}{2},H_2)$ $\rightarrow
  C_2$ hold where $\ppnt{q}{2} \subseteq \ppnt{q}{1}$ and $H_2 \subset
  H_1$ and $C_2 \in H_1$ are true. Then the D-sequent
  \oDs{\ppnt{q}{1}}{H_1 \setminus \s{C_2}}{C_1} holds.
\end{lemma}
%
\begin{mmproof}
  Assume that \V{F} are assigned as in \ppnt{q}{1} and clauses of $H_1
  \setminus \s{C_2}$ are not proved redundant yet. Let us show that
  \cof{(C_1)}{q_1} is redundant in \prob{X}{\cof{F}{q_1}} and so
  \oDs{\ppnt{q}{1}}{H_1 \setminus \s{C_2}}{C_1} holds. Consider the
  following two situations.  First, assume that clause $C_2$ is not
  proved redundant yet. Then the D-sequent \oDs{\ppnt{q}{q}}{H_1}{C_1}
  holds and so \cof{(C_1)}{q_1} is redundant in
  \prob{X}{\cof{F}{q_1}}.

  Now assume that clause $C_2$ is \ti{already proved} redundant.
  Denote D-sequents \oDs{\ppnt{q}{1}}{H_1}{C_1} and
  \oDs{\ppnt{q}{2}}{H_2}{C_2} by $S_1$ and $S_2$ respectively. Denote
  by $S^*_2$ the D-sequent used to prove redundancy of $C_2$. Let
  $S^*_2,Q_1,\dots,Q_p$ list the order in which $S^*_2$ and the
  following D-sequents are applied. Below, we show that one transform
  this consistent sequence of D-sequents into the sequence
  $Q_1,\dots,Q_p,S_1,S_2$. The latter sequence is also
  consistent and proves redundancy of clause $C_1$.

  First, note that one can replace $S^*_2$ with $S_2$ in the original
  sequence since clauses of $H_1 \setminus {C_1}$ are not proved
  redundant yet and $H_2 \subset H_1$ holds. For the same reason, one
  can replace sequence $S_2,Q_1,\dots,Q_p$ with
  $Q_1,\dots,Q_p,S_2$. Indeed, pushing $S_2$ forward cannot make a
  D-sequent $Q_i$ invalid $i=1,\dots,p$. Besides, $S_2$ is valid even
  after applying D-sequents $Q_1,\dots,Q_n$. Finally, one can insert
  D-sequent $S_1$ before $S_2$ to produce sequence
  $Q_1,\dots,Q_p,S_1,S_2$. Indeed, $S_1$ is still valid after applying
  $Q_1,\dots,Q_n$ and does not invalidate $S_2$.
\end{mmproof}
------
Finally,
Proposition~\ref{prop:red_add_cls} shows that a clause remains
redundant in \prob{X}{F} after adding clauses implied by $F$.
---------
%
%  Proposition: closed set of D-sequents
%
\begin{proposition}
%  \label{prop:closed_set}
  Let \prob{X}{F} be an \ecnf.  Let
  \oDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$,\oDs{\ppnt{q}{n}}{H_n}{C_n} be
  D-sequents where $H_i \subseteq \s{C_1,\dots,C_n}$ holds
  $i=1,\dots,n$. Then robust D-sequents \ooods{\ppnt{s}{1}}{C_1},
  $\dots$, \ooods{\ppnt{s}{n}}{C_n} hold where $\ppnt{s}{i}=
  \ppnt{q}{i} \cup \ppnt{q}{i_1} \cup \dots \ppnt{q}{i_p}$ and $H_i =
  \s{C_{i_1},\dots,C_{i_p}}$. (That is \ppnt{s}{i} is obtained by
  adding to \ppnt{q}{i} the conditionals of the D-sequents specifying
  the redundancy of clauses from $H_i$.)
\end{proposition}
%
\begin{mmproof}
  Let $S_i$ denote D-sequent
  \oDs{\ppnt{q}{i}}{H_i}{C_i},$i=1,\dots,n$.  Assume for the sake of
  simplicity that these D-sequents are applied in the order they are
  numbered $S_1,\dots,S_n$. Note that in this case $S_n$ has to be a
  robust D-sequent (i.e. $H_n = \emptyset$) because otherwise $S_n$
  would be invalidated by a previous D-sequent. For the same reason,
  the relations $H_{n-1} \subseteq \s{C_{n}}$, $H_{n-2} \subseteq
  \s{C_{n-1},C_n}$ and so on hold. To obtain robust D-sequents we
  iteratively apply Proposition~\ref{prop:subst}.

  First, we get rid of the presence of clause $C_n$ in sets
  $H_i$. Suppose, for instance, that $C_n$ is $H_i$. Then applying
  Proposition~\ref{prop:subst} to D-sequents $S_i$ and $S_n$ one can
  replace \oDs{\ppnt{q}{i}}{H_i}{C_i} with \oDs{\ppnt{q}{i} \cup
    \ppnt{q}{n}}{H_i \setminus \s{C_n}}{C_i}. After doing this for all
  D-sequents $S_i$ with $C_n \in H_i$ we obtain a new set of
  D-sequents $S_1,\dots,S_n$ with order constraits that do not include
  $C_n$. Note that after than D-sequent $S_{n-1}$ becomes robust. At
  this point we can use Proposition~\ref{prop:subst} to get rid of the
  presence of clause $C_{n-1}$ in the order constraints. Going on in
  such manner we will get the required set of robust D-sequents.  
\end{mmproof}
--------------
\begin{proposition}
  \label{prop:closed_set}
   Let \prob{X}{F} be an \ecnf.  Let
   \oDs{\ppnt{q}{1}}{H_1}{C_1},$\dots$,\oDs{\ppnt{q}{n}}{H_n}{C_n} be
   D-sequents where $H_i \subseteq \s{C_1,\dots,C_n}$ holds
   $i=1,\dots,n$. Then robust D-sequents \ooods{\ppnt{s}{1}}{C_1},
   $\dots$, \ooods{\ppnt{s}{n}}{C_n} hold where $\ppnt{s}{i}=
   \ppnt{q}{i} \cup \ppnt{q}{i_1} \cup \dots \ppnt{q}{i_p}$ and $H_i =
   \s{C_{i_1},\dots,C_{i_p}}$. (That is \ppnt{s}{i} is obtained by
   adding to \ppnt{q}{i} the conditionals of the D-sequents specifying
   the redundancy of clauses from $H_i$.)
\end{proposition}
--------
Assume that $H_2 \subset H_1$ holds. Then the D-sequent
\ods{q}{H}{C_1} of Proposition~\ref{prop:subst} is indeed less fragile
than \ods{q_1}{H_1}{C_1} since $H \subset H_1$ holds. The proposition
below shows how one can turn fragile D-sequents into robust ones.
-------------
To check if $S_1,\dots,S_k$ is indeed consistent one needs to apply
  the following procedure. Let $Q_1,\dots,Q_n$ is be the set of parent
  atomic D-sequents from which D-sequents $S_i$ have been
  obtained. Let $V$ by the set of variables on which D-sequents $Q_i$
  and their descendents have been joined to get D-sequents $S_i$. Then
  D-sequents $S_1,\dots,S_k$ are indeed inconsistent if there is an
  assignment to variables of $V$
------
%
% twin boundary points
%
\begin{lemma}
\label{lemma:twin_bnd_pnts}
Let \pnt{p} be a \s{v}-boundary point of CNF formula $G(Z)$ where $v
\in Z$.  Let \pnt{p'} be obtained from \pnt{p} by flipping the value
of $v$.  Then \pnt{p'} either satisfies $G$ or it is also a
\s{v}-boundary point of $G$.
\end{lemma}
\begin{mmproof}
Assume the contrary, \ie \pnt{p'} falsifies a clause $C$ of $G$ that
does not have a literal of $v$. (That is \pnt{p'} is neither a
satisfying assignment nor a \s{v}-boundary point of $G$.) Since
\pnt{p} is different from \pnt{p'} only in the value of $v$, it also
falsifies $C$. Then, since $v \not\in \V{C}$, \pnt{p} cannot be a
\s{v}-boundary point and we have a contradiction.
%$\square$
\end{mmproof}
----------
%
%  Subsection: joining D-sequents
%
\subsection{Joining D-sequents}
\label{ssec:join_oper}
----------
Let \prob{X}{F(X,Y} be an \ecnf and $C$ be an $X$-clause of $F$.  Let
\oods{r}{C} be a D-sequent and \pnt{q} be a branch of the search tree
such that $\pnt{r} \subseteq \pnt{q}$. Since this D-sequent has an
empty order constraint it can be used in branch \pnt{q} regardless of
what $X$-clauses of $F$ are currently proved redundant. For that
reason will refer to a D-sequent with a empty order constraint as
\tb{robust}.

Now suppose that \ods{r}{H}{C} be a D-sequent with a non-empty order
constraint $H$. This D-sequent cannot be used in the branch \pnt{q}
above if this order constraint is broken (i.e. if a clause $B \in H$
is already proved redundant). For that reason we will call such a
D-sequent \tb{fragile}. Intuitively, the larger $H$, the more fragile
this D-sequent is.
-----------
Propositions~\ref{prop:subst} below can be used to
make a D-sequent more robust.
-------------
We also recall the notion of composable D-sequents
presented in~\cite{fmcad13} and introduce a consistent set of
D-sequents (Subsection~\ref{ssec:cons_dseqs}). Finally, we show one
can ``align'' D-sequents computed with respect to different formulas
(Subsection~\ref{ssec:align}).
-----------
% Strengthening order constraint
%
\begin{proposition}
%  \label{prop:stren_order}
  Let \prob{X}{F} be an \ecnf. Let D-sequent \ods{q}{H}{C} hold. Let
  $R$ be an arbitrary subset of $X$-clauses of $F \setminus H$. Then
  D-sequent \ods{q}{H \cup R}{C} holds too.
\end{proposition}
%
--------
% proof
%
\begin{mmproof}
Denote $F \wedge R$ as $F'$.  Assume the contrary, \ie \cof{C}{q} is
redundant in \prob{X}{\cof{F}{q}} but not in \prob{X}{\cof{F'}{q}}.
The latter means that there is a boundary point \pnt{p} of $F'$ such
that \pnt{p} falsifies only clause \cof{C}{q} and \pnt{p} is
$X$-removable in \cof{F'}{q}.

Since \cof{C}{q} is in \cof{F}{q}, \pnt{p} is a boundary point of
\cof{F}{q} as well. Let us show that \pnt{p} is also $X$-removable in
\cof{F}{q}, which means that $C$ is not redundant in
\prob{X}{\cof{F}{q}} and we have a contradiction.  Assume the
contrary, i.e. \pnt{p} is not $X$-removable in \cof{F}{q}. Then there
is a point \pnt{s} satisfying \cof{F}{q} obtained from \pnt{p} by
flipping values of variables of $X$. Since $F \Rightarrow R$ holds,
\pnt{s} satisfies \cof{R}{q} too and hence it satisfies
\cof{F'}{q}. This contradicts the fact that \pnt{p} is $X$-removable
in \cof{F'}{q}.  $\square$
\end{mmproof}
--------
\begin{proposition}
%\label{prop:red_add_cls}
Let $X$-clause \cof{C}{q} be redundant in \prob{X}{\cof{F}{q}}. Let
$R$ be a CNF formula implied by $F$. Then \cof{C}{q} is redundant in
\prob{X}{\cof{F}{q} \wedge \cof{R}{q}} as well.
\end{proposition}
-------------
\begin{proposition}
\label{prop:elim_incr}
Let \prob{X}{F(X,Y)} be an \ecnf and \pnt{q} be an assignment to
variables of $F$.  Let \cof{H}{q} be a subset of $X$-clauses of
\cof{F}{q} redundant in \prob{X}{\cof{F}{q}}.  Let an $X$-clause
\cof{C}{q} of $\cof{F}{q} \setminus \cof{H}{q}$ be redundant in
\prob{X}{\cof{F}{q} \setminus \cof{H}{q}}. Then $\cof{H}{q} \cup
\s{\cof{C}{q}}$ is redundant in \prob{X}{\cof{F}{q}}.
\end{proposition}
----------
A similar approach can be used to solve the PQE problem of taking
formula $F_1$ out of the scope of quantifiers in \prob{X}{F_1(X,Y)
  \wedge F_2(X,Y)}. In this case, one just needs to eliminate the
$X$-removable boundary points falsifying only $X$-clauses of $F_1$.
----------------
The proofs are given in the
appendix\footnote{Proposition~\ref{prop:rem_bnd_pnt} was actually
  proved in~\cite{fmsd14}. For the sake of convenience, we reproduce
  the proof in question in the appendix}.
  -----------
Let $C$ be a clause, $H$ be a formula that may have quantifiers, and
\pnt{p} be an assignment. \cof{C}{p} is true if $C$ is satisfied by
\pnt{p}; otherwise it is the clause obtained from $C$ by removing all
literals falsified by \pnt{p}.  \cof{H}{p} denotes the formula
obtained from $H$ by removing every clause $C \in H$ for which
\cof{C}{p}=true and replacing $C$ with \cof{C}{p} if $\cof{C}{p} \neq
\mi{true}$.  In the context of this paper, it is convenient to assume
that clause \cof{C}{q} equal to \ti{true} remains in \cof{H}{q} rather
than being removed from \cof{H}{q}.  We treat such a clause as
\ti{redundant} in \cof{H}{q} (see Proposition~\ref{prop:sat_cls}).
--------


==> old_files/t0ransform_dseqs.tex <==
%\section{A Few Useful Procedures For Transforming D-sequents}
\section{Two Useful Transformations Of D-sequents}
\label{sec:trans_dseqs}
In this section, we describe two transformations that are useful for a
QE-solver based on the machinery of D-sequents. Since a QE-solver has
to add new clauses once in a while, D-sequents of different branches
are, in general, computed with respect to different formulas.  In
Subsection~\ref{ssec:align}, we describe a transformation meant for
``aligning'' such D-sequents. In Subsection~\ref{ssec:mak_rob}, we
describe a transformation meant for relaxing the order constraint of a
D-sequent. In Section~\ref{sec:dcds_plus}, this transformation is used
to generate a consistent set of D-sequents.

%
% Subsection: D-sequent alignment
%
\subsection{D-sequent alignment}
\label{ssec:align}
According to Definition~\ref{def:dseq}, a D-sequent holds with respect
to a particular \ecnf formula \prob{X}{F}.
Proposition~\ref{prop:dseq_add_cls} shows that this D-sequent also
holds after adding to $F$ implied clauses.
%
%  Proposition: D-sequent still holds after adding implications
%
\begin{proposition}
\label{prop:dseq_add_cls}
Let D-sequent \Ods{X}{F}{q}{H}{C} hold and $R$ be a CNF formula
implied by $F$. Then D-sequent \Ods{X}{F \wedge R}{q}{H}{C} holds too.
\end{proposition}

Proposition~\ref{prop:dseq_add_cls} is useful in aligning D-sequents
derived in different branches. Suppose that \Ods{X}{F}{q'}{H'}{C} is
derived in the current branch of the search tree where the last
assignment is $v=0$. Suppose that \Ods{X}{F \wedge R}{q''}{H''}{C} is
derived after flipping the value of $v$ from 0 to 1. Here $R$ is the
set of clauses implied by $F$ that has been added to $F$ before the
second D-sequent was derived.  One cannot apply the join operation to
these D-sequents because they are computed with respect to different
formulas. Proposition~\ref{prop:dseq_add_cls} allows one to replace
\Ods{X}{F}{q'}{H'}{C} with \Ods{X}{F\wedge R}{q'}{H'}{C}. The latter
can be joined with \Ods{X}{F\wedge R}{q''}{H''}{C} at variable $v$.

%
% Subsection: Making D-sequent more robust
%
\subsection{Making a D-sequent more robust}
\label{ssec:mak_rob}
In this subsection, we give two propositions showing how one can make
a D-sequent $S$ more robust. Proposition~\ref{prop:subst} introduces a
transformation that removes a clause from the order constraint of $S$
possibly adding to the latter some other
clauses. Proposition~\ref{prop:mak_rob} describes a scenario where by
repeatedly applying this transformation one can remove a clause from
the order constraint of $S$ \ti{without} adding any other clauses.

%
% Proposition: subsitutution
%
\begin{proposition}
  \label{prop:subst}  
Let \prob{X}{F} be an \ecnf.  Let \oDs{\pnt{q'}}{H'}{C'} and
$(\pnt{q''},H'')$$\rightarrow C''$ be two D-sequents forming a
consistent set (see Definition~\ref{def:cons_dseqs}). Let $C''$ be in
$H'$. Then  D-sequent \ods{q}{H}{C'} holds where $\pnt{q} =
\pnt{q'} \cup \pnt{q''}$ and $H = (H' \setminus \s{C''}) \cup H''$.
\end{proposition}



%
%  Proposition: making D-sequent more robust
%
\begin{proposition}
\label{prop:mak_rob}
Let \prob{X}{F} be an \ecnf and $(\ppnt{q}{1},H_1)$ $\rightarrow
C_1$,$\dots$, $(\ppnt{q}{k},H_k)$$\rightarrow C_k$ be consistent
D-sequents where $H_i \subseteq \s{C_1,\dots,C_k}$,
$i=1,\dots,k$. Assume, for the sake of simplicity, that the numbering
order is consistent with the order constraints. Let $C_m$ be in $H_i$.
Then, by repeatedly applying the transformation of
Proposition~\ref{prop:subst}, one can produce D-sequent \ods{q}{H_i
  \setminus \s{C_m}}{C_i} where $\ppnt{q}{i}~\subseteq~\pnt{q}
\subseteq \ppnt{q}{i} \cup \bigcup\limits_{j=m}^{j=k} \ppnt{q}{j}$.
\end{proposition}



==> old_files/t1ransform_dseqs_proofs.tex <==
\section*{Propositions of
  Section~\ref{sec:trans_dseqs}: Two Useful Transformations Of D-sequents}
%
% Lemma: used to prove that one can add implications
%
\begin{lemma}
\label{lem:mk_sat}
Let \prob{X}{F(X,Y)} be an \ecnf formula. Let \pnt{q} be an assignment
to \V{F}. Let $C$ be an $X$-clause redundant in \prob{X}{\cof{F}{q}}.
Let $C$ be also redundant in formula \prob{X}{\cof{W}{q}} where $W$ is
obtained from $F$ by dropping $X$-clauses that are redundant in
\prob{X}{\cof{F}{q}}. Then every point \pnt{p} falsifying only clause
\cof{C}{q} of \cof{W}{q} can be turned into a point satisfying $F$ by
changing values of (some) variables of $X$.
\end{lemma}
%
%
\begin{mmproof}
Denote by $C_1,\dots,C_k$ the $X$-clauses dropped from $F$ to obtain
$W$. Assume that these clauses were dropped in the numbering
order. That is clause $C_i$ is redundant in \prob{X}{W_i} in subspace
\pnt{q} where $W_1$ = $F$ and $W_{i+1} = W_i \setminus \s{C_i}$,
$i=1,\dots,k$. So $W_{k+1} = F \setminus \s{C_1,\dots,C_k} = W$.

Let \pnt{p} be a point falsifying only $C$ of $W$ in subspace
\pnt{q}. Since clause $C$ is redundant, one can turn \pnt{p}
into a point satisfying $W$ in subspace \pnt{q} by changing
values of variables of $X$. Denote the new point as \pnt{p}
again. If \pnt{p} satisfies $F$ then we are done. Otherwise,
\pnt{p} falsifies some clauses $C_1,\dots,C_k$.

Let $C_i$ be the clause with the largest index that is falsified by
\pnt{p}. Note that \pnt{p} falsifies only clause $C_i$ in $W_i$ in
subspace \pnt{q}. Since $C_i$ is redundant in \prob{X}{W_i} in
subspace \pnt{q}, one can turn \pnt{p} \,into an assignment satisfying
$W_i$ in subspace \pnt{q} \,by changing only assignments to $X$. Denote
the new point as \pnt{p} again. If \pnt{p} satisfies $F$ we are
done. Otherwise, \pnt{p} falsifies some clauses $C_1,\dots,C_{i-1}$.

Going on in such a manner one eventually builds a point satisfying $F$
that is obtained from the very first point \pnt{p} by changing only
assignments to variables of $X$.  $\square$
\end{mmproof}

%
%  Proposition: D-sequent still holds after adding implications
%
\begin{proposition}
 %\label{prop:dseq_add_cls}
Let D-sequent \Ods{X}{F}{q}{H}{C} hold and $R$ be a CNF formula
implied by $F$. Then D-sequent \Ods{X}{F \wedge R}{q}{H}{C} holds too.
\end{proposition}
%
\begin{mmproof}
Let $W^R$ be a member formula for \Ods{X}{F \wedge R}{q}{H}{C}.
Denote by $W$ the formula $W^R \setminus R$. Note that $W$ is a member
formula for \Ods{X}{F}{q}{H}{C}. If $W = W^R$, then $C$ is redundant
in \prob{X}{W} (and hence in \prob{X}{W^R}) in subspace \pnt{q}.  Now
consider the case $W \subset W^R$. Assume that $C$ is not redundant in
\prob{X}{W^R} in subspace \pnt{q}. Then there is a point \pnt{p} such
that
\begin{itemize}
\item \pnt{p} falsifies only clause $C$ of $W_R$ in subspace \pnt{q}
  where $\pnt{q} \subseteq \pnt{p}$
\item \pnt{p} is $X$-removable for every \pnt{r} obtained from \pnt{q}
  \,by dropping (some) assignments to $X$.
\end{itemize}
Since $C$ is redundant in \prob{X}{W} in subspace \pnt{q}, from
Lemma~\ref{lem:mk_sat}, it follows that one can turn \pnt{p} into
point \pnt{p^*} satisfying $F$ by changing only values of variables of
$X$. Since $R$ is implied by $F$, \pnt{p^*} satisfies $F \wedge R$ as
well. Hence \pnt{p^*} satisfies $W_R$ and \pnt{p} is not $X$-removable
in subspace \pnt{r} obtained by dropping from \pnt{q} all assignments
to $X$. So we have a contradiction.  $\square$
\end{mmproof}
%
% Lemma: two redundant clauses
%
\begin{lemma}
\label{lem:two_red_cls}
Let \prob{X}{F} be an \ecnf formula and \pnt{q} be an assignment to
\V{F}. Let $C'$ and $C''$ be $X$-clauses of $F$ and \s{C',C''} be
redundant in \prob{X}{F} in subspace \pnt{q}. Then clause $C'$ is
redundant in \prob{X}{F \setminus \s{C''}} in subspace \pnt{q}.
\end{lemma}
\begin{mmproof}
Assume that $C'$ is not redundant in \prob{X}{F \setminus \s{C''}}.
in subspace \pnt{q}. Then there is a point \pnt{p} falsifying only
\cof{C'}{q} that is $X$-removable in every subspace $\pnt{q^*}
\subseteq \pnt{r} \subseteq \pnt{q}$ (see
Definition~\ref{def:virt_red}). Then, from
Proposition~\ref{prop:red_cls_set} it follows that clauses \s{C',C''}
are not redundant in \prob{X}{F} in subspace \pnt{q} (even virtually).  $\square$
\end{mmproof}

%
% Lemma: subsitutution
%
\begin{lemma}
  \label{lem:subst}
  Let \prob{X}{F} be an \ecnf. Let D-sequents \ods{q'}{H'}{C'} and
  $(\pnt{q''},H'')$ $\rightarrow C''$ hold where $\pnt{q''} \subseteq
  \pnt{q'}$ and $H'' \subset H'$ and $C'' \in H'$ and $C' \not\in
  H''$. Then the D-sequent \ods{q'}{H' \setminus \s{C''}}{C'} holds.
\end{lemma}
%
\begin{mmproof}
  Let $W$ be a member formula for \ods{q'}{H' \setminus
    \s{C''}}{C'}. Let us show that $C'$ is redundant in \prob{X}{W} in
  subspace \pnt{q'} and so \ods{q'}{H' \setminus \s{C''}}{C'}
  holds. Consider the following two situations.  First, assume that
  clause $C'' \in W$. Then $W$ is a member formula for the D-sequent
  \ods{q'}{H'}{C'} and hence $C'$ is redundant in \prob{X}{W} in
  subspace \pnt{q'}.

  Now assume that clause $C'' \not\in W$.  Denote D-sequents
  \ods{q'}{H'}{C'} and \ods{q'}{H''}{C''} (computed with respect to
  \prob{X}{F}) as $S'$ and $S''$ respectively. Denote formula $W \cup
  \s{C''}$ by $W''$. Note that $W''$ is a member formula for $S'$ and
  $S''$. Besides, $S'$ and $S''$ are consistent. So, in particular,
  $S''$ can be used after $S'$ . By applying $S'$ and $S''$ one shows
  that \s{C',C''} are redundant in \prob{X}{W''} in subspace
  \pnt{q'}. From Lemma~\ref{lem:two_red_cls} it follows that $C'$ is
  redundant in \prob{X}{W} in subspace \pnt{q'}.  $\square$
\end{mmproof}

%
% Lemma: strengthen order constraint
%
\begin{lemma}
  \label{lem:stren_order}
  Let \prob{X}{F} be an \ecnf. Let D-sequent \ods{q}{H}{C} hold. Let
  $G$ be an arbitrary subset of $X$-clauses of $F \setminus H$. Then
  D-sequent \ods{q}{H \cup G}{C} holds too.
\end{lemma}
%
\begin{mmproof}
Let $W$ be a member formula for \ods{q}{H \cup G}{C}. Then $W$ is a
member formula for \ods{q}{H}{C}. So, $C$ is redundant in \prob{X}{W}
in subspace \pnt{q}.~$\square$
\end{mmproof}
%
% Proposition: subsitutution
%
\begin{proposition}
% \label{prop:subst}
Let \prob{X}{F} be an \ecnf.  Let \oDs{\pnt{q'}}{H'}{C'} and
$(\pnt{q''},H'')$$\rightarrow C''$ be two D-sequents forming a
consistent set (see Definition~\ref{def:cons_dseqs}). Let $C''$ be in
$H'$. Then  D-sequent \ods{q}{H}{C'} holds where $\pnt{q} =
\pnt{q'} \cup \pnt{q''}$ and $H = (H' \setminus \s{C''}) \cup H''$.
\end{proposition}
%
\begin{mmproof}
  From Proposition~\ref{prop:subspace} it follows that D-sequent
  \ods{q}{H'}{C'} holds. From Lemma~\ref{lem:stren_order} it follows
  that \ods{q}{H' \cup H''}{C'} holds too. The latter and D-sequent
  \ods{q''}{H''}{C''} satisfy the conditions of
  Lemma~\ref{lem:subst}. (Note that $H''$ cannot contain $C'$ because
  \ods{q'}{H'}{C'} and $(\pnt{q''},H'')$ $\rightarrow C''$ are
  consistent.)  This entails that \ods{q}{H}{C'} holds.  $\square$
\end{mmproof}

%
%  Proposition: making D-sequent more robust
%
\begin{proposition}
%\label{prop:mak_rob}
Let \prob{X}{F} be an \ecnf and $(\ppnt{q}{1},H_1)$ $\rightarrow
C_1$,$\dots$, $(\ppnt{q}{k},H_k)$$\rightarrow C_k$ be consistent
D-sequents where $H_i \subseteq \s{C_1,\dots,C_k}$,
$i=1,\dots,k$. Assume, for the sake of simplicity, that the numbering
order is consistent with the order constraints. Let $C_m$ be in $H_i$.
Then, by repeatedly applying the transformation of
Proposition~\ref{prop:subst}, one can produce D-sequent \ods{q}{H_i
  \setminus \s{C_m}}{C_i} where $\ppnt{q}{i}~\subseteq~\pnt{q}
\subseteq \ppnt{q}{i} \cup \bigcup\limits_{j=m}^{j=k} \ppnt{q}{j}$.
\end{proposition}
%
\begin{mmproof}
 Let $S_j$ denote D-sequent \oDs{\ppnt{q}{j}}{H_j}{C_j},
 $j=1,\dots,k$. Note that $i < m$ holds, otherwise, $S_m$ would be
 used before $S_i$ proving $C_m$ redundant and thus making $S_i$
 inapplicable.  Let us use Proposition~\ref{prop:subst} to remove
 clause $C_m$ from the order constraint of $S_m$. This produces a new
 D-sequent $S$ equal to \nods{q}{(H_i \cup H_m) \setminus
   \s{C_m}}{C_i} where $\pnt{q} = \ppnt{q}{i} \cup \ppnt{q}{m}$.  If
 $H_m \subseteq H_i$ holds, the proposition in question is
 proved. Otherwise, one keeps removing clauses from the order
 constraint of D-sequent $S$.

 Let $C_r$ be the clause of $H_m \setminus H_i$ with the largest
 index. Note that $m < r$ holds (and, hence, $i < m < r$) for the same
 reason $i < m$ does.  By applying Proposition~\ref{prop:subst} to
 remove clause $C_r$ from the order constraint of $S$ one produces a
 new D-sequent $S$ equal to \ods{q}{(H_i \cup H_m \cup H_r) \setminus
   \s{C_m,C_r}}{C_i} where $\pnt{q} = \ppnt{q}{i} \cup \ppnt{q}{m}
 \cup \ppnt{q}{r}$. Note that since $i < r$ and $m < r$, set $H_r$
 cannot contain $C_m$ or $C_r$.  If $(H_m \cup H_r) \setminus \s{C_r}$
 is a subset of $H_i$ the proposition in question is
 proved. Otherwise, one picks the clause of $(H_m \cup H_r) \setminus
 \s{C_r}$ with the largest index that is not in $H_i$ and removes it
 by applying the transformation of Proposition~\ref{prop:subst}.

 The procedure above goes one until one produces a D-sequent $S$ with
 order constraint $H_i \setminus \s{C_m}$. This procedure converges,
 since one always removes a clause with the largest index and so this
 clause cannot re-appear in the order constraint of $S$. Thus,
 eventually, in no more than $k-m$ steps, all the clauses that are not
 in $H_i \setminus \s{C_{m}}$ will be removed from the order
 constraint of $S$.  $\square$
\end{mmproof}


==> old_files/v0irt_redund.tex <==
\section{Virtual redundancy}
\label{sec:virt_red}

If a boundary point \pnt{p} is $X$-removable in \prob{X}{\cof{F}{q}},
this does not mean that it is $X$-removable in \prob{X}{F} (see
Remark~\ref{rem:no_reverse}). This fact leads to the following
problem.  Let \pnt{q} and \pnt{r} be two assignments to \V{F} and
$\pnt{q} \subset \pnt{r}$.  Suppose that clause $C$ is redundant in
\prob{X}{F} in subspace \pnt{q}. It is natural to expect that this
also holds in the smaller subspace \pnt{r}. However,
$\prob{X}{\cof{F}{q}} \equiv \prob{X}{\cof{F}{q} \setminus
  \cof{C}{q}}$ does not imply $\prob{X}{\cof{F}{r}} \equiv
\prob{X}{\cof{F}{r} \setminus \cof{C}{r}}$. In particular, due to this
problem, one cannot define the join operation in terms of redundancy
specified by Definition~\ref{def:red_cls}. To address this issue we
introduce the notion of \ti{virtual} redundancy.
%
%  Definition
%
\begin{definition}
\label{def:virt_red}
Let \prob{X}{F(X,Y)} be an \ecnf formula, \pnt{q} be an assignment
to \V{F}, and \cof{C}{q} be an $X$-clause of \cof{F}{q}. Let $B$ be
the set of points of $F$ such every $\pnt{p} \in B$ falsifies only
clause $C$ and is $X$-removable. Clause \cof{C}{q} is called
\tb{virtually redundant} in \prob{X}{\cof{F}{q}} if one of the two
conditions are true.
\begin{enumerate}
\item $B = \emptyset$ or
\item For every $\pnt{p} \in B$, there is an assignment \pnt{r} where
  $\pnt{q^*} \subseteq \pnt{r} \subset \pnt{q}$ such that \pnt{p} is
  \ti{not} $X$-removable in \cof{F}{r}. Here \pnt{q^*} is obtained
  from \pnt{q} by removing all value assignments to variables of $X$.
\end{enumerate}
\end{definition}

The first condition just means that $\prob{X}{\cof{F}{q} \setminus
  \cof{C}{q}} \equiv \prob{X}{\cof{F}{q}}$.  We will refer to this
type of redundancy (earlier specified by Definition~\ref{def:red_cls})
as \ti{regular} redundancy. Regular redundancy is a special case of
virtual redundancy.


%
%  Proposition: about a subspace
%
\begin{proposition}
\label{prop:subspace}
Let \pnt{q} be an assignment to \V{F} and clause \cof{C}{q} be
redundant in \prob{X}{\cof{F}{q}}. Then, for every \pnt{r} such that
$\pnt{q} \subset \pnt{r}$, clause \cof{C}{r} is virtually redundant in
\prob{X}{\cof{F}{r}}.
\end{proposition}

From now on, when we say that a clause \cof{C}{r} is redundant in
\prob{X}{\cof{F}{r}} we mean that it is at least \ti{virtually
  redundant}. Note that, in general, proving virtual redundancy of $C$
in subspace \pnt{r} can be extremely hard. We avoid this problem by
using the notion of virtual of redundancy only if we have \ti{already
  proved} that $C$ is redundant in a subspace containing subspace
\pnt{r}. (For instance, we have already proved that $C$ is redundant
in \prob{X}{F} in subspace \pnt{q} where $\pnt{q} \subset \pnt{r}$.)


==> old_files/v1irt_redund_proofs.tex <==
\section*{Propositions of Section~\ref{sec:virt_red}: Virtual Redundancy}
%
%  Proposition: about a subspace
%
\begin{proposition}
  %\label{prop:subspace}
Let \pnt{q} be an assignment to \V{F} and clause \cof{C}{q} be
redundant in \prob{X}{\cof{F}{q}}. Then, for every \pnt{r} such that
$\pnt{q} \subset \pnt{r}$, clause \cof{C}{r} is virtually redundant in
\prob{X}{\cof{F}{r}}.
\end{proposition}
%
\begin{mmproof}
  Let a point \pnt{p} of $F$ falsify only \cof{C}{r} and be
  $X$-removable.  Then \pnt{p} falsifies only clause \cof{C}{q} of
  \cof{F}{q}.  Since \cof{C}{q} is redundant in \prob{X}{\cof{F}{q}},
  point \pnt{p} \,is not $X$-removable in \cof{F}{q}. $\square$
\end{mmproof}

